Warping the Edge: Where Instant Mobility in 5G Meets Stateful Applications

Edge computing is considered a key paradigm for supporting real-time applications over 5G networks, as hosting applications at the network edge can substantially reduce delays. A significant fraction of real-time applications over 5G are expected to be highly mobile applications. However, one challenge with hosting mobile applications on the network edge is ensuring that users continue to get low latency as they move across different locations. This requires the support to handover clients to different edge sites with negligible application delays. However, many edge applications are stateful and can experience significant downtime during state migration over 5G. This paper addresses the problem of enabling stateful mobile edge applications in 5G networks. We first identify the key architectural issues and then propose a new system design, EdgeWarp, that mitigates delays during mobility through proactive application state migration. To enable this, we extend the existing edge data stores with the design of a novel two-step application state synchronization protocol, that leverages the early prediction of the target edge host. Additionally, EdgeWarp prioritizes the handover of latency-sensitive edge applications by communicating their latency requirements to the 5G control plane at the beginning of a data session. Our evaluation with real edge applications shows up to a 15.4x reduction in application downtime under mobility. We have made our anonymized code publicly accessible here.

==> abstract_old.tex <==
Edge computing is considered a key paradigm for supporting real-time applications over 5G networks, as hosting applications at the network edge can substantially reduce delays. A significant fraction of real-time applications over 5G are expected to be highly mobile applications, e.g., safety applications for connected cars, real-time mapping and localization, and mobile AR/VR. However, one challenge with hosting mobile applications on the network edge is ensuring that users continue to get low latency as they move across different locations.  This in turn requires the support to handover clients to different edge sites with negligible delays. However, migrating \textit{stateful applications} over 5G can cause significant application downtime. This paper considers the problem of enabling stateful mobile edge applications over 5G networks. We identify the key architectural issues and propose a new systems architecture, EdgeCat, to address them.
EdgeCat mitigates delays during mobility through proactive application state migration. To enable this, we extend the existing data stores with our proposed design to facilitate two-step application state synchronization based on the early prediction of the target edge host by utilizing the radio network information. Additionally, EdgeCat prioritizes the handover of latency-sensitive edge applications by communicating their latency requirements to the 5G control plane at the beginning of a data session.
Our evaluation with real edge applications shows up to a 15.4$\times$ reduction in application downtime under mobility. We have made our anonymized code publicly accessible here.


==> conclusion.tex <==
\section{Conclusion}
\label{conclusion}
5G networks aim to support edge applications that require time-bound guarantees on their packet processing. Existing approaches fail to provide such latency guarantees during control plane faults. \Name enables 5G to cope with control plane faults to ensure these applications achieve their delay budgets. 
\Name uses multiple active control plane clones at the edge to speedup the control plane operations and consequently reduce application delays. This approach addresses slow failure detection in \ExistingSystems, and masks the impact of straggler nodes. \Name implements a custom quorum protocol which provides consistency guarantees for both deterministic and non-deterministic control plane operations. 


% 5G systems design supports latency sensitive applications that require time-bound guarantees on their packet processing. Existing approaches fail to provide such latency guarantees during failure. \Name enables 5G to cope with different failure use cases while ensuring applications achieve their stringent latency requirements. 
% \Name implements a custom quorum-based protocol in which the user's control messages are multicast to a quorum of control plane functions. This approach addresses slow failure detection during failure, and mitigates the impact of straggler nodes. It provides consistency guarantees for both deterministic and non-deterministic control plane operations. 

==> design.tex <==
\section{Design}
\label{sec:design}
% To address the issues in \S\ref{challenges}, we design a new system architecture, \Name. \Name is a cross-layer design that (a) exposes low-level network information (e.g., radio link quality information reported by the mobile client to the base station) to edge apps so they can proactively perform application state migration, and (b) shares application requirements (e.g. whether the app is latency-sensitive) with the 5G control plane for speeding 5G handovers. 
To address the issues in \S\ref{challenges}, we design a new system architecture, \Name. \Name is a cross-layer design that (a) exposes radio network information (reported by the UE to the base station) through the MEC APIs~\cite{5g_mec_rni1} to edge apps so they can proactively perform application state migration, and (b) shares application latency requirements with the 5G control plane for speeding 5G handovers. 
\Name consists of three new modules: (i) a module for proactively predicting target base stations for mobile clients (\S\ref{sec:design:target_bs_predction}), (ii) an edge data store for stateful edge apps that can leverage proactive network information to speed up application state synchronization (\S\ref{sec:design_app_state_migration}), and (iii) app-aware control plane for speeding up 5G handover events (\S\ref{sec:app_impact_on_control_plane}). In this section, we first discuss our goasl and assumptions in designing \Name (\S\ref{sec:goals_and_assumptions}), then provide an overview of our proposed architecture (\S\ref{sec:design:system_architecture}), before discussing the individual modules in detail. 


% Talk about MEC and new interfaces
%We discuss target base prediction in \S\ref{sec:design:target_bs_predction}, extended edge data store design \S\ref{sec:design_app_state_migration} and an app-aware control plane design in section \S\ref{sec:app_impact_on_control_plane}.
% Too many bullets
% Do we need to discuss about the 


\subsection{Goals and Assumptions}
\label{sec:goals_and_assumptions}

The key goal of \Name is to  \textit{\underline{reduce app downtime} for stateful edge apps when migrating application state due to client mobility}. At the same time, \Name aims to incur minimal latency and bandwidth overheads in non-mobility scenarios. We next make explicit our assumptions about the deployment and computational model before diving into our design.

\begin{itemize}[leftmargin=*]
    \item We assume edge deployment of the cellular core network which is the preferred deployment option for latency-sensitive apps \cite{iot_in_5g_era_cisco, ericsson_e2e_network_slices}.
   \item We assume a client-server model for apps. An app server hosted at the network edge provides services to mobile clients. A stateful app server maintains per-user app state.
   \item To make our design discussion concrete, we assume edge apps are hosted at every BS. Our design can be generalized for other less extreme edge deployments where the app can be hosted at any aggregation point between the BS and remote cloud \cite{mec_in_5g}.
   \item We assume edge apps require strict consistency which implies \textit{when a user connects to a target edge app instance, it will see exactly the same app state for the user as it was before the handover at the source edge app instance}. A system designed for strict consistency can be easily tuned for apps that can tolerate relaxed consistency models \cite{tanenbaum}.

\end{itemize}

\begin{comment}
% \subsection{Design Overview}
% \label{sec:desing_overview}

% Below we provide an overview of the key ideas in \Name:
% \begin{itemize}[leftmargin=*]
%     \setlength{\itemsep}{0pt}
%     \setlength{\parskip}{0pt}
    
%     \item \textbf{Proactive app state migration: } \Name provides a mechanism for proactive App state migration before a 5G handover starts. If naively done, it can introduce significant overhead. For instance, latency-sensitive Apps typically have high update rates (e.g., online games can have $\approx$100 updates/s~\cite{zhang2017towards_online_game_updates_rate}) and if the App state is always replicated on some target host, it can introduce significant bandwidth overhead. \Name starts proactive app state migration just before a 5G handover starts. To enable this, \Name uses the following key ideas.   
%     \begin{itemize}
%     \item \textit{Target BS prediction}: \Name predicts target BS before a 5G handover starts. We call it a mobility hint. The mobility hint provides an opportunity window to proactively synchronize all or a subset of the app state with the target edge host~(\S\ref{sec:design:target_bs_predction}).
    
%     \item \textit{Edge data store assisted two-step state synchronization}: \Name modifies the existing edge data stores (e.g., \redis and \memcache) to track the app dynamic state and perform two-step state syncing. To enable this, the modified  external data store tracks the update rate of every state variable from the set/update requests toward the data store. \Name leverages the mobility hint to perform two-step state syncing. The first step spans from a mobility hint to the start of a 5G handover during which background state syncing is performed. The second step spans from the start of a 5G handover until the user's complete App state is synced with the target edge host. The external data store performs blocking state synchronization during the second step as the App won't receive any updates from UE during a 5G handover~(\S\ref{sec:design_app_state_migration}).
    
%     \end{itemize}
    
%     \item \textbf{App-aware control plane processing: } Control plane in \Name can significantly reduce 5G handover completion time for the latency-sensitive edge Apps. To enable this, \Name exposes new APIs (table~\ref{tab:api_for_app_influence_on_cpf}) to latency-sensitive edge Apps to register themselves for priority processing. The new APIs are exposed to the app server only to avoid misuse of client apps registering themselves for priority processing. As a trade-off, it can slow down control plane operations for delay-tolerant {users} which is an acceptable trade-off  \cite{latency_nbiot_catm, iot_in_5g_era_cisco, 3gpp_evaluation_mmtc}~(\S\ref{sec:app_impact_on_control_plane}).
% \end{itemize}
    
% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{figs/system_architecture_diagram.png}
% \vspace{-0.3in}
% \caption{\Name's (\underline{EdgeCat}alyst) system architecture.}
% % .\fawad{Except in the first para of 4.1, there are no references to this figure}}
% \vspace{-0.3in}
% \label{fig:system_architecture_diagram}
% \end{figure}


%  \noindent\textbf{Resultant Architecture:}
%  Figure~\ref{fig:system_architecture_diagram} shows \Name's high-level system architecture. Our design is based on stateless edge Apps where the user's App state is stored in a fast local edge data store.
%  % \fawad{Stateless or stateful?} 
%  The edge data store exposes new APIs~(table~\ref{tab:api_in_edge_store}) to the edge Apps to perform two-step App state synchronization. The target BS predictor module receives real-time RNI and other mobility-related events by using the APIs available to the edge Apps in 5G \cite{5g_mec_rni1, mec_apis_combined}. The target BS predictor module predicts the destination BS in advance before an actual handover starts. The mobility handler module takes into account the target BS and provides target edge host and App instance information (such as IP address, port number, etc.) to the local app to facilitate proactive App state migration. The app-aware cellular control plane exposes new APIs~(table~\ref{tab:api_for_app_influence_on_cpf}) to edge Apps to prioritize their control plane processing.
\end{comment}


\subsection{\Name's System Architecture}
\label{sec:design:system_architecture}

Figure~\ref{fig:system_architecture_diagram} provides an overview of \Name's system architecture. \Name argues to store the user's app state in our modified edge data store while the application logic is stateless.
To enable this, the modified data store exposes new APIs (Table~\ref{tab:api_in_edge_store}) to applications. The target BS predictor module receives real-time radio network information (RNI) exposed to applications in 5G \cite{5g_mec_rni1, mec_apis_combined} and predicts the destination BS in advance before an actual handover starts. The mobility handler module receives information about the target BS from the target BS predictor module and provides the target edge host and application instance information (such as IP address, port number, etc.) to the source app instance to facilitate proactive application state migration. The app-aware cellular control plane leverages the application-level information (such as latency needs) to provide priority processing for latency-sensitive edge apps. To enable this, the app-aware cellular control plane exposes new APIs~(Table~\ref{tab:api_for_app_influence_on_cpf}) to edge apps to prioritize their control plane processing. 


\begin{figure}
\centering
\includegraphics[width=0.7\columnwidth]{figs/system_architecture_diagram.png}
\vspace{-0.3in}
\caption{\Name's system architecture.}
% \vspace{-0.3in}
\label{fig:system_architecture_diagram}
\end{figure}


\subsection{Target BS Prediction}
\label{sec:design:target_bs_predction}

\Name tries to predict the target BS  before a handover decision and relays this information to the mobility handler module (Figure~\ref{fig:system_architecture_diagram}) to facilitate proactive app state migration. For this purpose, \Name implements a 2-step target BS prediction pipeline as depicted in Figure \ref{fig:target_bs_prediction_architecture}. \Name's target BS prediction is based on RNI APIs which expose  near real-time radio signal measurements reported to the BS  by the UE, such as Reference Signal Received Power (RSRP) and Reference Signal Received Quality (RSRQ) \cite{rsrp_rsrq}. 

\noindent{\textbf{Handover Prediction:}}
 We use \circled{1} a handover prediction module to trigger the target BS prediction module. The purpose of the handover prediction module is to avoid target BS prediction when no handover is going to take place. We leverage a recent work, Prognos~\cite{hassan2022vivisecting}, for handover prediction. Prognos predicts a handover through a pattern of LTE/5G radio measurement events~\cite{5g_nr_measurement_events}. A  limitation of Prognos is that it can forecast a handover but cannot predict the specific target BS. We use Prognos as it provides reasonably good accuracy (i.e., F1-score 0.92–0.94~\cite{hassan2022vivisecting}) but it can be replaced by any other handover prediction module in our pipeline.

\noindent{\textbf{Target BS Prediction:}}
The most essential component of our target BS prediction pipeline is a Long Short Term Memory (LSTM) recurrent neural network. On a handover prediction, \circled{2a} the binary LSTM classifier predicts the probable target BSs, and \circled{2b} the conflict resolver module determines a single target BS out of multiple candidate BSs. Input to the LSTM network is a feature vector (shown in Figure~\ref{fig:feature_Vector}) comprising a configurable number of both absolute and relative values of the RSRP and RSRQ. The binary LSTM network classifies all pairs of source and target BSs for which the UE reports measurements. Out of multiple possible target BSs predicted by the LSTM network, the conflict resolver module selects one BS with the highest probability of handover to avoid state syncing with multiple target BSs. %We train our LSTM network on multiple 5G/4G radio network traces collected in high-speed trains~\cite{hst_sigcomm_dataset}, driving tests~\cite{incp_dataset}, and other miscellaneous mobility scenarios~\cite{mobile_insight_logs}~(\S\ref{appendix_dataset_description}). 
Our target BS prediction pipeline is co-located with the edge apps on the edge site to avoid network delays.

\begin{figure}
\centering
\includegraphics[width=0.7\columnwidth]{figs/target_bs_prediction.png}
\vspace{-0.3in}
\caption{\Name's target BS prediction pipeline.}
\vspace{-0.2in}
\label{fig:target_bs_prediction_architecture}
\end{figure}

\subsection{Two-Step App State Synchronization}
\label{sec:design_app_state_migration}

In this section, we discuss our modifications to the existing data stores to provide two-step state synchronization based on mobility hints. 

\noindent{\textbf{Modification to Data Store:}} Our modifications to the data store include keeping an additional meta-state with every key to track whether a state object is updated after the previous synchronization event and sorting state objects based on their update rates. The additional per-key meta-state in the data store at the source edge host includes:
\begin{itemize}[leftmargin=*]
    \item \textit{First update time}: The time the key was created in the  data store.

    \item \textit{Last update time}: The time when the key was last time updated in the data store.

    \item \textit{Updates count}: The total number of key updates.

    \item \textit{Last sync time}: The time when the key was last synced with the data store instance at the target edge host. To avoid any conflict when an update and sync operation are performed in parallel, the external data store records the time before the sync process starts for a key (say T) and updates T as the last sync time when the sync operation successfully completes.
\end{itemize}


The meta-state gives useful information about (i) the  average key update rate and (ii) whether the key is updated after the last sync. We leverage the per-key meta-state to define additional APIs (in Table \ref{tab:api_in_edge_store}) in the modified data store. 


\noindent{\textbf{Background State Synchronization:}} An edge app registers itself with the mobility handler module (Figure~\ref{fig:system_architecture_diagram}) to receive important network events, such as mobility hint and mobility handover. The mobility handler module receives target BS information from the target BS prediction module and provides destination edge host and app instance information (i.e., IP address, port number) to the source edge app.
On reception of a mobility hint, the source edge app calls \textit{BackgroundSync} API exposed by our modified data store. %The source edge app calls \textit{BackgroundSync} API with the destination edge host information received from the mobility handler module. 
Call to the \textit{BackgroundSync} API initiates the syncing of the user's app state with the target data store instance by synchronizing the state object that has the lowest update rate and was updated after the last sync event (update time higher than sync time).
%(with lower chances of being updated before a handover) and updated after the last sync (update time higher than sync time). 
The background syncing blocks updates to the key only when getting a copy of the state. The migration and restoration in the target data store instance is a non-blocking operation. As read operations are very fast in edge-suitable data stores (such as \redis and \memcache), this allows the application to process users' requests with minimal overhead during background state syncing.

\noindent{\textbf{Blocking State Synchronization:}} 
On a 5G handover signal from the mobility handler module, the source edge app calls \textit{BlockingSync} API in Table \ref{tab:api_in_edge_store} by providing it with a callback function. This API synchronizes the rest of the state that is either not synced or updated after the last sync. In the best case scenario, all the user's application state is migrated during the background syncing and the callback function returns right after the call to the \textit{BlockingSync} API. In the worse case, all the user's application state needs to be synced due to post-sync updates. The duration from call to  \textit{BlockingSync} API to the callback call is the blocking state migration time---also the minimum app downtime during an app handover. If the third parameter (retain) in \textit{BlockingSync} API is true, the source data store instance will not delete the user state otherwise it will be deleted after the migration completes.


% \begin{table}
% \parbox{.38\linewidth}{
% \centering
% \begin{tabular}{| c |} 
% \hline
%     \textbf{New APIs in Modified Data Store}\\
%     \hline
%     \textit{BackgroundSync (userID, destHost)}\\
%     \hline
%     \textit{BlockingSync (userID, callBackFunc, retain)}\\
%     \hline
% \end{tabular}
% \caption{Foo}
% }
% \hfill
% \parbox{.55\linewidth}{
% \centering
% \begin{tabular}[\columnwidth]{| c| c |} 
%     \hline
%     NF & \textbf{New APIs for AF}\\
%     \hline
%     AMF & \textit{Set\_Priority (IpAddress, priority)}\\
%     \hline
%     AMF & \textit{Revert\_Priority (IpAddress)}\\
%     \hline
%     RAN & \textit{Set\_Priority (RAN UE NG-AP ID, priority)}\\
%     \hline
%     RAN & \textit{Revert\_Priority (RAN UE NG-AP ID)}\\
%     \hline
% \end{tabular}
% \caption{Bar}
% }
% \end{table}

\begin{table}
\caption{New APIs for latency-sensitive edge apps in the modified data store tailored to the needs of latency-sensitive mobile applications.}
\vspace{-0.15in}
\begin{center}
\begin{tabular}{| c| c |} 
\hline
    \textbf{Sr. \#} &\textbf{New APIs introduced in modified data store}\\
    \hline
    1 & \textit{BackgroundSync (userID, destinationEdgeHost)}\\
    \hline
    2 & \textit{BlockingSync (userID, callBackFunction, retain)}\\
    \hline
\end{tabular}
\vspace{-0.2 in}

\label{tab:api_in_edge_store}
\end{center}
\end{table}


\subsection{App-Aware Control Plane Processing}
\label{sec:app_impact_on_control_plane}
In this section, we discuss how an AMF can differentiate between different types of UEs. We also describe how an AMF leverages this information to perform priority processing for the UEs running a latency-sensitive app session.

\noindent{\textbf{5G Services Classes:}} 5G networks are aiming to support three broad classes of services, (i) enhanced Mobile Broad Band (eMBB), (ii) Ultra-Reliable and Low Latency Communication (URLLC), and (iii) delay-tolerant low-complexity Massive IoT (MIoT) \cite{3gpp_architecture, latency_nbiot_catm, iot_in_5g_era_cisco,critical_iot, 3gpp_evaluation_mmtc}.

\noindent{\textbf{UE Classes at AMF:}}
 An AMF can differentiate between the low-complexity (MIoT) and other (eMBB \& URLLC) devices from the information provided by RAN or UE.\footnote{UE context at AMF (table 5.2.2.2.2-1 of the 3GPP document~\cite{3gpp_23_502}) contains information if a UE is a low-complexity device such NB-IoT, LTE-M or RedCap (reduced capability device). Section 1.8 of the 3GPP document~\cite{3gpp_124_008_nas_low_priority_info} suggests a UE can explicitly inform the core network that it is a low-priority device.} An AF, on the behalf of app~\cite{mec_in_5g}, can inform which eMBB or URLLC device is to be treated normally or with high priority by the control plane. 
% When a UE starts a data session with a latency-sensitive edge App, AF informs the AMF (through a PCF or NEF \cite{3gpp_architecture}) to perform control plane operations for the UE with the highest priority. On session termination, the AF informs the AMF to remove the UE from the high-priority list. 
% Table \ref{tab:api_for_app_influence_on_cpf} shows the APIs exposed to the AF to set a priority level for a UE on the AMF and RAN.
In the context of delay tolerance, our modified AMF can differentiate between the following classes of UEs:


\begin{enumerate}[leftmargin=*]
    \item {\lowPriorityIot:} These are delay-tolerant low-complexity devices such as those used for smart cities, e.g., smart meters. A delay of up to 10\,s is acceptable for these UEs \cite{latency_nbiot_catm, iot_in_5g_era_cisco, 3gpp_evaluation_mmtc}. \Name's AMF is configured to have \textit{lowest priority} for such UEs.
    \item {\mediumPriorityIot:} 
    Includes the rest of devices not included in \lowPriorityIot, such as eMBB and URLLC.
    % Represents the class of UEs requiring lower latency than the \lowPriorityIot, whose requirements are generally met in existing networks but degradation in the quality of service may impact their performance. 
    Such UEs are typically used in agriculture, education, and media production, etc \cite{iot_in_5g_era_cisco, cellular_iot_ericsson}. Voice services can also be included in this class of UEs. These UEs have \textit{medium priority} in \Name. 
    \item {\highPriorityIot:} These are devices from the \mediumPriorityIot having an active latency-sensitive data session with an edge app. These UEs have deadlines in the order of few ms \cite{critical_iot, iot_in_5g_era_cisco}. Autonomous vehicles \cite{self_driving_cars_lin2018architectural} and VR headsets \cite{vr-latency} are key examples of such UEs. A UE is only added to this class when an eMBB or URLLC device starts a latency-sensitive data session with an edge app. These UEs have \textit{highest priority} in \Name.
\end{enumerate}



\noindent\textbf{{Priority Processing for Latency-Sensitive Apps:}}
We leverage the UE class information at the AMF to perform priority processing for latency-sensitive apps at RAN and AMF. Radio Resource Control (RRC) layer~\cite{3gpp_architecture} provides a control plane signaling protocol between a UE and RAN. We maintain three separate priority queues for the RRC messages at the BS. The Next Generation Application Protocol (NG-AP) provides the control plane signaling protocol between the RAN and AMF. We maintain three priority queues at the BS for the NG-AP messages from the AMF. Similarly, we maintain three queues at the AMF from the control messages received from the BS. UEs at the RAN and AMF are identified with their unique IDs, \textit{RAN UE NGAP ID} and \textit{AMF UE NGAP ID}, respectively.
 The priority levels are configurable in our design and can be updated by network operators based on their preferences.\footnote{The control processing threads at the BS and AMF by default process 6/10, 3/10, and 1/10 control messages from \highPriorityIot, \mediumPriorityIot, and \lowPriorityIot queues, respectively.} If a high-priority queue is empty, we process messages from one level lower priority queue. Our design requires no changes at the UE. In section \S\ref{appendix_d}, we provide a detailed discussion of the sequence of steps involved when an edge app calls the APIs in Table~\ref{tab:api_for_app_influence_on_cpf} to prioritize their processing.
 

\definecolor{yellow}{RGB}{244,240,236}
\definecolor{pink}{RGB}{255, 255, 240}

\begin{table}
\caption{New APIs available in \Name for an AF to influence control plane operations at the RAN and AMF.}
\vspace{-0.15in}
\begin{center}
\begin{tabular}[\columnwidth]{| c| c |} 
    \hline
    NF & \textbf{New APIs available for App Function (AF)}\\
    \hline
    AMF & \textit{Set\_Priority (IpAddress, priorityLevel)}\\
    \hline
    AMF & \textit{Revert\_Priority (IpAddress)}\\
    \hline
    RAN & \textit{Set\_Priority (RAN UE NG-AP ID, priorityLevel)}\\
    \hline
    RAN & \textit{Revert\_Priority (RAN UE NG-AP ID)}\\
    \hline
\end{tabular}
\vspace{-0.1 in}

\label{tab:api_for_app_influence_on_cpf}
\end{center}
\end{table}




==> design_v1.tex <==
\section{Design}
\label{sec:design}
To address the issues in \S\ref{challenges}, we design a new system architecture, \Name. \Name is a cross-layer design that (a) exposes radio network information (reported by the UE to the BS) through the MEC APIs~\cite{5g_mec_rni1} to edge apps so they can proactively perform application state migration, and (b) shares application latency requirements with the 5G control plane for speeding 5G handovers. 
\Name consists of three new modules: (i) a module for proactively predicting target BSs for mobile clients (\S\ref{sec:design:target_bs_predction}), (ii) an edge data store for stateful edge apps that can leverage proactive network information to speed up application state synchronization (\S\ref{sec:design_app_state_migration}), and (iii) app-aware control plane for speeding up 5G handover events (\S\ref{sec:app_impact_on_control_plane}). In this section, we first discuss our goals and assumptions in designing \Name (\S\ref{sec:goals_and_assumptions}), then provide an overview of our proposed architecture (\S\ref{sec:design:system_architecture}), before discussing the individual modules in detail. 


\subsection{Goals and Assumptions}
\label{sec:goals_and_assumptions}

The key goal of \Name is to  \textit{\underline{reduce app downtime} for stateful edge apps when migrating application state due to client mobility}. At the same time, \Name aims to incur minimal latency and bandwidth overheads in non-mobility scenarios. We next make explicit our assumptions about the deployment and computational model before diving into our design.

\begin{itemize}[leftmargin=*]
    \item We assume edge deployment of the cellular core network which is the preferred deployment option for latency-sensitive apps \cite{iot_in_5g_era_cisco, ericsson_e2e_network_slices}.
   \item We assume a client-server model for apps. An app server hosted at the network edge provides services to mobile clients. A stateful app server maintains a per-user app state.
   \item To make our design discussion concrete, we assume edge apps are hosted at every BS. Our design can be generalized for other less extreme edge deployments where the app can be hosted at any aggregation point between the BS and remote cloud \cite{mec_in_5g}.
   \item We assume edge apps require strict consistency which implies \textit{when a user connects to a target edge app instance, it will see exactly the same app state for the user as it was before the handover at the source edge app instance}. A system designed for strict consistency can be easily tuned for apps that can tolerate relaxed consistency models \cite{tanenbaum}.

\end{itemize}

\subsection{\Name's System Architecture}
\label{sec:design:system_architecture}

Figure~\ref{fig:system_architecture_diagram} provides an overview of \Name's system architecture. \Name argues to store the user's app state in our modified edge data store while the application logic is stateless.
To enable this, the modified data store exposes new APIs (Table~\ref{tab:api_in_edge_store}) to applications. The target BS predictor module receives real-time radio network information (RNI) exposed to applications in 5G \cite{5g_mec_rni1, mec_apis_combined} and predicts the destination BS in advance before an actual handover starts. The mobility handler module receives information about the target BS from the target BS predictor module and provides the target edge host and application instance information (such as IP address, port number, etc.) to the source app instance to facilitate proactive application state migration. The app-aware cellular control plane leverages the application-level information (such as latency needs) to provide priority processing for latency-sensitive edge apps. To enable this, the app-aware cellular control plane exposes new APIs~(Table~\ref{tab:api_for_app_influence_on_cpf}) to edge apps to prioritize their control plane processing. 


% \begin{figure}
% \centering
% \includegraphics[width=0.7\columnwidth]{figs/system_architecture_diagram.png}
% \vspace{-0.3in}
% \caption{\Name's system architecture.}
% % \vspace{-0.3in}
% \label{fig:system_architecture_diagram}
% \end{figure}


\subsection{Target BS Prediction}
\label{sec:design:target_bs_predction}

\Name tries to predict the target BS  before a handover decision and relays this information to the mobility handler module (Figure~\ref{fig:system_architecture_diagram}) to facilitate proactive app state migration. For this purpose, \Name implements a 2-step target BS prediction pipeline as shown in Figure~\ref{fig:target_bs_prediction_architecture}. \Name's target BS prediction is based on RNI APIs which expose  near real-time radio signal measurements reported to the BS  by the UE, such as Reference Signal Received Power (RSRP) and Reference Signal Received Quality (RSRQ) \cite{rsrp_rsrq}. 

\noindent{\textbf{Handover Predictor:}} Every UE is configured to initiate reporting of the signal strength of neighboring BSs when the signal strength of the source BS deteriorates beyond a preconfigured threshold~\cite{5g_nr_measurement_events}. These reports include RSRP and RSRQ. \circled{1} Our handover prediction is based on a Long Short-Term Memory (LSTM) recurrent neural network (\S\ref{appendix_lstm_binary_classifier}). We use an LSTM network due to (i) temporal trends in the measurement reports and (ii) to avoid per-user data storage required for history-based BS prediction~\cite{bs_prediction_ho_history}. Our LSTM network predicts the probability of handover from the source BS to each neighboring BS for which radio measurements have been reported. The input to the LSTM network is a feature vector (discussed in section~\ref{appendix_lstm_binary_classifier}) consisting of a configurable number of absolute and relative values of the RSRP and RSRQ. The binary LSTM network classifies all pairs of source and target BSs based on the reported measurements from the UE. When the handover probability from the source BS to any target BS exceeds a threshold (let's say it is $P_{t}$) learned from the data, it indicates that a handover is likely to occur.

\noindent{\textbf{Conflict Resolver:}}
When a handover is likely to occur, there may be multiple BSs with a probability of handover exceeding the threshold $P_{t}$. \circled{2} Among the multiple potential target BSs predicted by the LSTM network, the conflict resolver module determines the top-x target BSs from the pool of candidate BSs.\footnote{Here, x is a configurable number, typically set as 1, but it can be adjusted to meet the specific requirements of edge apps.}.
To minimize network delays, our target BS prediction pipeline is deployed alongside the edge applications at the edge site.

% \begin{figure}
% \centering
% \includegraphics[width=0.7\columnwidth]{figs/target_bs_prediction.png}
% \vspace{-0.2in}
% \caption{\Name's target BS prediction pipeline.}
% \vspace{-0.3in}
% \label{fig:target_bs_prediction_architecture}
% \end{figure}


\begin{figure}[tb]
\centering
\begin{minipage}[t]{0.57\linewidth}
\includegraphics[width=\columnwidth]{figs/system_architecture_diagram.png}
\vspace{-0.3in}
\caption{\Name's system architecture.}
% \vspace{-0.3in}
\label{fig:system_architecture_diagram}
\end{minipage} 
\vspace{-0.15 in}
\hfill%
\begin{minipage}[t]{0.38\linewidth}
\includegraphics[width=\columnwidth]{figs/target_bs_prediction_upldated.png}
\vspace{-0.3in}
\caption{\Name's target BS prediction pipeline.}
\vspace{-0.1in}
\label{fig:target_bs_prediction_architecture}
\end{minipage}%
\end{figure}


\subsection{Two-Step Application State Synchronization}
\label{sec:design_app_state_migration}

In this section, we discuss our modifications to the existing data stores to provide two-step state synchronization based on mobility hints. 

\noindent{\textbf{Modification to Data Store:}} Our modifications to the data store include keeping an additional meta-state with every key to track whether a state object is updated after the previous synchronization event and sorting state objects based on their update rates. The additional per-key meta-state in the data store at the source edge host includes:
\begin{itemize}[leftmargin=*]
    \item \textit{First update time}: The time the key was created in the  data store.

    \item \textit{Last update time}: The time when the key was last time updated in the data store.

    \item \textit{Updates count}: The total number of key updates.

    \item \textit{Last sync time}: The time when the key was last synced with the data store instance at the target edge host. To avoid any conflict when an update and sync operation are performed in parallel, the external data store records the time before the sync process starts for a key (say T) and updates T as the last sync time when the sync operation successfully completes.
\end{itemize}


The meta-state gives useful information about (i) the  average key update rate and (ii) whether the key is updated after the last sync. We leverage the per-key meta-state to define additional APIs (in Table \ref{tab:api_in_edge_store}) in the modified data store. 


\noindent{\textbf{Background State Synchronization:}} An edge app registers itself with the mobility handler module (Figure~\ref{fig:system_architecture_diagram}) to receive important network events, such as mobility hint and mobility handover. The mobility handler module receives target BS information from the target BS prediction module and provides destination edge host and app instance information (i.e., IP address, port number) to the source edge app.
On reception of a mobility hint, the source edge app calls \textit{BackgroundSync} API exposed by our modified data store.
Call to the \textit{BackgroundSync} API initiates the syncing of the user's app state with the target data store instance by synchronizing the state object that has the lowest update rate and was updated after the last sync event (update time higher than sync time).
The background syncing blocks updates to the key only when getting a copy of the state. The migration and restoration in the target data store instance is a non-blocking operation. As read operations are very fast in edge-suitable data stores (such as \redis and \memcache), this allows the application to process users' requests with minimal overhead during background state syncing.

\noindent{\textbf{Blocking State Synchronization:}} 
On a 5G handover signal from the mobility handler module, the source edge app calls \textit{BlockingSync} API in Table \ref{tab:api_in_edge_store} by providing it with a callback function. This API synchronizes the rest of the state that is either not synced or updated after the last sync. In the best case scenario, all the user's application state is migrated during the background syncing and the callback function returns right after the call to the \textit{BlockingSync} API. In the worse case, all the user's application state needs to be synced due to post-sync updates. The duration from call to  \textit{BlockingSync} API to the callback call is the blocking state migration time---also the minimum app downtime during an app handover. If the third parameter (retain) in \textit{BlockingSync} API is true, the source data store instance will not delete the user state otherwise it will be deleted after the migration completes.


\begin{table}
\parbox{0.4\columnwidth}{
\centering
\begin{tabular}{| c |} 
\hline
    \textbf{New APIs in Modified Data Store}\\
    \hline
    \textit{BackgroundSync (userID, destHost)}\\
    \hline
    \textit{BlockingSync (userID, callBackFunc, retain)}\\
    \hline
\end{tabular}
\caption{New APIs for latency-sensitive edge apps in the modified data store tailored to the needs of latency-sensitive mobile applications.}
\label{tab:api_in_edge_store}
}
\hfill
\parbox{.52\columnwidth}{
\centering
\begin{tabular}[\columnwidth]{| c| c |} 
    \hline
    NF & \textbf{New APIs for Application Function}\\
    \hline
    AMF & \textit{Set\_Priority (IpAddress, priority)}\\
    \hline
    AMF & \textit{Revert\_Priority (IpAddress)}\\
    \hline
    RAN & \textit{Set\_Priority (RAN UE NG-AP ID, priority)}\\
    \hline
    RAN & \textit{Revert\_Priority (RAN UE NG-AP ID)}\\
    \hline
\end{tabular}
\caption{New APIs available in \Name for an AF to influence control plane operations at the RAN and AMF.}
\label{tab:api_for_app_influence_on_cpf}
}
\vspace{-0.4in}
\end{table}


\subsection{App-Aware Control Plane Processing}
\label{sec:app_impact_on_control_plane}
In this section, we discuss how an AMF can differentiate between different types of UEs. We also describe how an AMF leverages this information to perform priority processing for the UEs running a latency-sensitive app session.

\noindent{\textbf{5G Services Classes:}} 5G networks are aiming to support three broad classes of services, (i) enhanced Mobile Broad Band (eMBB), (ii) Ultra-Reliable and Low Latency Communication (URLLC), and (iii) delay-tolerant low-complexity Massive IoT (MIoT) \cite{3gpp_architecture, latency_nbiot_catm, iot_in_5g_era_cisco,critical_iot, 3gpp_evaluation_mmtc}.

\noindent{\textbf{UE Classes at AMF:}}
 An AMF can differentiate between the low-complexity (MIoT) and other (eMBB \& URLLC) devices from the information provided by RAN or UE.\footnote{UE context at AMF (table 5.2.2.2.2-1 of the 3GPP document~\cite{3gpp_23_502}) contains information if a UE is a low-complexity device such NB-IoT, LTE-M or RedCap (reduced capability device). Section 1.8 of the 3GPP document~\cite{3gpp_124_008_nas_low_priority_info} suggests a UE can explicitly inform the core network that it is a low-priority device.} An AF, on behalf of app~\cite{mec_in_5g}, can inform which eMBB or URLLC device is to be treated normally or with high priority by the control plane. 
In the context of delay tolerance, our modified AMF can differentiate between the following classes of UEs:


\begin{enumerate}[leftmargin=*]
    \item {\lowPriorityIot:} These are delay-tolerant low-complexity devices such as those used for smart cities, e.g., smart meters. A delay of up to 10\,s is acceptable for these UEs \cite{latency_nbiot_catm, iot_in_5g_era_cisco, 3gpp_evaluation_mmtc}. \Name's AMF is configured to have \textit{lowest priority} for such UEs.
    \item {\mediumPriorityIot:} 
    Includes the rest of devices not included in \lowPriorityIot, such as eMBB and URLLC.
    Such UEs are typically used in agriculture, education, media production, etc \cite{iot_in_5g_era_cisco, cellular_iot_ericsson}. Voice services can also be included in this class of UEs. These UEs have \textit{medium priority} in \Name. 
    \item {\highPriorityIot:} These are devices from the \mediumPriorityIot having an active latency-sensitive data session with an edge app. These UEs have deadlines in the order of few ms \cite{critical_iot, iot_in_5g_era_cisco}. Autonomous vehicles \cite{self_driving_cars_lin2018architectural} and VR headsets \cite{vr-latency} are key examples of such UEs. A UE is only added to this class when an eMBB or URLLC device starts a latency-sensitive data session with an edge app. These UEs have \textit{highest priority} in \Name.
\end{enumerate}



\noindent\textbf{{Priority Processing for Latency-Sensitive Apps:}}
We leverage the UE class information at the AMF to perform priority processing for latency-sensitive apps at RAN and AMF. Radio Resource Control (RRC) layer~\cite{3gpp_architecture} provides a control plane signaling protocol between a UE and RAN. We maintain three separate priority queues for the RRC messages at the BS. The Next Generation Application Protocol (NG-AP) provides the control plane signaling protocol between the RAN and AMF. We maintain three priority queues at the BS for the NG-AP messages from the AMF. Similarly, we maintain three queues at the AMF from the control messages received from the BS. UEs at the RAN and AMF are identified with their unique IDs, \textit{RAN UE NGAP ID} and \textit{AMF UE NGAP ID}, respectively.
 The priority levels are configurable in our design and can be updated by network operators based on their preferences.\footnote{The control processing threads at the BS and AMF by default process 6/10, 3/10, and 1/10 control messages from \highPriorityIot, \mediumPriorityIot, and \lowPriorityIot queues, respectively.} If a high-priority queue is empty, we process messages from one level lower priority queue. Our design requires no changes at the UE. In section \S\ref{appendix_d}, we provide a detailed discussion of the sequence of steps involved when an edge app calls the APIs in Table~\ref{tab:api_for_app_influence_on_cpf} to prioritize their processing.





==> design_v2.tex <==
\section{Design}
\label{sec:design}
To address the issues in \S\ref{challenges}, we design a new system architecture, \Name. \Name is a cross-layer design that (a) exposes radio network information (reported by the UE to the BS) through the MEC APIs~\cite{5g_mec_rni1} to edge apps so they can proactively perform application state migration, and (b) shares application latency requirements with the 5G control plane for speeding 5G handovers. 
\Name consists of three new modules: (i) a module for proactively predicting target BSs for mobile clients (\S\ref{sec:design:target_bs_predction}), (ii) an edge data store for stateful edge apps that can leverage proactive network information to speed up application state synchronization (\S\ref{sec:design_app_state_migration}), and (iii) app-aware control plane for speeding up 5G handover events (\S\ref{sec:app_impact_on_control_plane}). In this section, we first discuss our goals and assumptions in designing \Name (\S\ref{sec:goals_and_assumptions}), then provide an overview of our proposed architecture (\S\ref{sec:design:system_architecture}), before discussing the individual modules in detail. 


\subsection{Goals and Assumptions}
\label{sec:goals_and_assumptions}

The key goal of \Name is to  \textit{\underline{reduce app downtime} for stateful edge apps when migrating application state due to client mobility}. At the same time, \Name aims to incur minimal latency and bandwidth overheads in non-mobility scenarios. We next make explicit our assumptions about the deployment and computational model before diving into our design.

\begin{itemize}[leftmargin=*]
    \item We assume edge deployment of the cellular core network which is the preferred deployment option for latency-sensitive apps \cite{iot_in_5g_era_cisco, ericsson_e2e_network_slices}.
   \item We assume a client-server model for apps. An app server hosted at the network edge provides services to mobile clients. A stateful app server maintains a per-user app state.
   \item To make our design discussion concrete, we assume edge apps are hosted at every BS. Our design can be generalized for other less extreme edge deployments where the app can be hosted at any aggregation point between the BS and remote cloud \cite{mec_in_5g}.
   \item We assume edge apps require strict consistency which implies \textit{when a user connects to a target edge app instance, it will see exactly the same app state for the user as it was before the handover at the source edge app instance}. A system designed for strict consistency can be easily tuned for apps that can tolerate relaxed consistency models \cite{tanenbaum}.

\end{itemize}

\subsection{\Name's System Architecture}
\label{sec:design:system_architecture}

Figure~\ref{fig:system_architecture_diagram} provides an overview of \Name's system architecture. \Name argues to store the user's app state in our modified edge data store while the application logic is stateless.
To enable this, the modified data store exposes new APIs (Table~\ref{tab:api_in_edge_store}) to applications. The target BS predictor module receives real-time radio network information (RNI) exposed to applications in 5G \cite{5g_mec_rni1, mec_apis_combined} and predicts the destination BS in advance before an actual handover starts. The mobility handler module receives information about the target BS from the target BS predictor module and provides the target edge host and application instance information (such as IP address, port number, etc.) to the source app instance to facilitate proactive application state migration. The app-aware cellular control plane leverages the application-level information (such as latency needs) to provide priority processing for latency-sensitive edge apps. To enable this, the app-aware cellular control plane exposes new APIs~(Table~\ref{tab:api_for_app_influence_on_cpf}) to edge apps to prioritize their control plane processing. 


% \begin{figure}
% \centering
% \includegraphics[width=0.7\columnwidth]{figs/system_architecture_diagram.png}
% \vspace{-0.3in}
% \caption{\Name's system architecture.}
% % \vspace{-0.3in}
% \label{fig:system_architecture_diagram}
% \end{figure}


\subsection{Target BS Prediction}
\label{sec:design:target_bs_predction}

\Name tries to predict the target BS  before a handover decision and relays this information to the mobility handler module (Figure~\ref{fig:system_architecture_diagram}) to facilitate proactive app state migration. For this purpose, \Name implements a multi-step target BS prediction pipeline as shown in Figure~\ref{fig:target_bs_prediction_architecture}. \Name's target BS prediction is based on RNI APIs which expose  near real-time radio signal measurements reported to the BS  by the UE, such as Reference Signal Received Power (RSRP) and Reference Signal Received Quality (RSRQ) \cite{rsrp_rsrq}. The target BS prediction pipeline works as follows.

\begin{enumerate}[leftmargin=*]
\item Our target BS prediction is based on an LSTM network (section~\ref{appendix_lstm_binary_classifier}) to account for temporal trends in measurement reports and avoid per-user data storage required for history-based BS prediction~\cite{bs_prediction_ho_history}. The LSTM network predicts the handover probability from the source BS to each neighboring BS having enough samples for prediction. It utilizes a feature vector (section \ref{appendix_lstm_binary_classifier}) comprising a configurable number (N, default value set to 6 based on evaluation results) of absolute and relative values of RSRP and RSRQ. The binary LSTM network classifies all source and target BS pairs based on reported measurements from the UE.
% \item Our target BS prediction is based on a Long Short-Term Memory (LSTM) recurrent neural network (\S\ref{appendix_lstm_binary_classifier}) due to (i) temporal trends in the measurement reports and (ii) to avoid per-user data storage required for history-based BS prediction~\cite{bs_prediction_ho_history}. Our LSTM network predicts the probability of handover from the source BS to each neighboring BS for which radio measurements have been reported. The input to the LSTM network is a feature vector (\S\ref{appendix_lstm_binary_classifier}) consisting of a configurable number (let's say N, with default value 6 based on our evaluation results) of absolute and relative values of the RSRP and RSRQ. The binary LSTM network classifies all pairs of source and target BSs based on the reported measurements from the UE.

    \item When the handover probability from the source BS to any target BS exceeds a learned threshold (denoted as $P_{t}$, with a learned value of 0.37), it indicates a high likelihood of a handover.

    \item When a handover is likely, predicting the actual target BS becomes crucial. However, during the handover prediction, there is a possibility of missing the actual target BS if it has fewer than N samples available at that stage. To address this, we extrapolate the RSRP and RSRQ values by a single sample for BSs that have N - 1 samples reported. We avoid extrapolating multiple samples to prevent errors caused by transient radio fluctuations.

    \item  If a single extrapolation process has generated the required number of samples (N) for any new BS, we apply an LSTM classifier on the new pair of source and potential target BS.

    \item Among the multiple potential target BSs predicted by the LSTM network (at steps 1 and 4), the conflict resolver module determines the top-x target BSs from the pool of candidate BSs---x is a configurable number, typically set as 1, but it can be adjusted to meet the specific requirements of edge apps.

\end{enumerate}

To minimize network delays, our target BS prediction pipeline is deployed alongside the edge apps at the edge site.

% \noindent{\textbf{Handover Predictor:}} Every UE is configured to initiate reporting of the signal strength of neighboring BSs when the signal strength of the source BS deteriorates beyond a preconfigured threshold~\cite{5g_nr_measurement_events}. These reports include RSRP and RSRQ. \circled{1} Our handover prediction is based on a Long Short-Term Memory (LSTM) recurrent neural network (\S\ref{appendix_lstm_binary_classifier}). We use an LSTM network due to (i) temporal trends in the measurement reports and (ii) to avoid per-user data storage required for history-based BS prediction~\cite{bs_prediction_ho_history}. Our LSTM network predicts the probability of handover from the source BS to each neighboring BS for which radio measurements have been reported. The input to the LSTM network is a feature vector (discussed in section~\ref{appendix_lstm_binary_classifier}) consisting of a configurable number of absolute and relative values of the RSRP and RSRQ. The binary LSTM network classifies all pairs of source and target BSs based on the reported measurements from the UE. When the handover probability from the source BS to any target BS exceeds a threshold (let's say it is $P_{t}$) learned from the data, it indicates that a handover is likely to occur.

% \noindent{\textbf{Conflict Resolver:}}
% When a handover is likely to occur, there may be multiple BSs with a probability of handover exceeding the threshold $P_{t}$. \circled{2} Among the multiple potential target BSs predicted by the LSTM network, the conflict resolver module determines the top-x target BSs from the pool of candidate BSs.\footnote{Here, x is a configurable number, typically set as 1, but it can be adjusted to meet the specific requirements of edge apps.}.
% To minimize network delays, our target BS prediction pipeline is deployed alongside the edge applications at the edge site.

% \begin{figure}
% \centering
% \includegraphics[width=0.7\columnwidth]{figs/target_bs_prediction.png}
% \vspace{-0.2in}
% \caption{\Name's target BS prediction pipeline.}
% \vspace{-0.3in}
% \label{fig:target_bs_prediction_architecture}
% \end{figure}


\begin{figure}[tb]
\centering
\begin{minipage}[t]{0.57\linewidth}
\includegraphics[width=\columnwidth]{figs/system_architecture_diagram.png}
\vspace{-0.3in}
\caption{\Name's system architecture.}
% \vspace{-0.3in}
\label{fig:system_architecture_diagram}
\end{minipage} 
\vspace{-0.15 in}
\hfill%
\begin{minipage}[t]{0.3\linewidth}
\includegraphics[width=\columnwidth]{figs/target_bs_prediction_upldated.png}
\vspace{-0.3in}
\caption{\Name's target BS prediction pipeline.}
\vspace{-0.1in}
\label{fig:target_bs_prediction_architecture}
\end{minipage}%
\end{figure}


\subsection{Two-Step Application State Synchronization}
\label{sec:design_app_state_migration}

In this section, we discuss our modifications to the existing data stores to provide two-step state synchronization based on mobility hints. 

\noindent{\textbf{Modification to Data Store:}} Our modifications to the data store include keeping an additional meta-state with every key to track whether a state object is updated after the previous synchronization event and sorting state objects based on their update rates. The additional per-key meta-state in the data store at the source edge host includes:
\begin{itemize}[leftmargin=*]
    \item \textit{First update time}: The time the key was created in the  data store.

    \item \textit{Last update time}: The time when the key was last time updated in the data store.

    \item \textit{Updates count}: The total number of key updates.

    \item \textit{Last sync time}: The time when the key was last synced with the data store instance at the target edge host. To avoid any conflict when an update and sync operation are performed in parallel, the external data store records the time before the sync process starts for a key (say T) and updates T as the last sync time when the sync operation successfully completes.
\end{itemize}


The meta-state gives useful information about (i) the  average key update rate and (ii) whether the key is updated after the last sync. We leverage the per-key meta-state to define additional APIs (in Table \ref{tab:api_in_edge_store}) in the modified data store. 


\noindent{\textbf{Background State Synchronization:}} An edge app registers itself with the mobility handler module (Figure~\ref{fig:system_architecture_diagram}) to receive important network events, such as mobility hint and mobility handover. The mobility handler module receives target BS information from the target BS prediction module and provides destination edge host and app instance information (i.e., IP address, port number) to the source edge app.
On reception of a mobility hint, the source edge app calls \textit{BackgroundSync} API exposed by our modified data store.
Call to the \textit{BackgroundSync} API initiates the syncing of the user's app state with the target data store instance by synchronizing the state object that has the lowest update rate and was updated after the last sync event (update time higher than sync time).
The background syncing blocks updates to the key only when getting a copy of the state. The migration and restoration in the target data store instance is a non-blocking operation. As read operations are very fast in edge-suitable data stores (such as \redis and \memcache), this allows the application to process users' requests with minimal overhead during background state syncing.

\noindent{\textbf{Blocking State Synchronization:}} 
On a 5G handover signal from the mobility handler module, the source edge app calls \textit{BlockingSync} API in Table \ref{tab:api_in_edge_store} by providing it with a callback function. This API synchronizes the rest of the state that is either not synced or updated after the last sync. In the best case scenario, all the user's application state is migrated during the background syncing and the callback function returns right after the call to the \textit{BlockingSync} API. In the worse case, all the user's application state needs to be synced due to post-sync updates. The duration from call to  \textit{BlockingSync} API to the callback call is the blocking state migration time---also the minimum app downtime during an app handover. If the third parameter (retain) in \textit{BlockingSync} API is true, the source data store instance will not delete the user state otherwise it will be deleted after the migration completes.


\begin{table}
\parbox{0.4\columnwidth}{
\centering
\begin{tabular}{| c |} 
\hline
    \textbf{New APIs in Modified Data Store}\\
    \hline
    \textit{BackgroundSync (userID, destHost)}\\
    \hline
    \textit{BlockingSync (userID, callBackFunc, retain)}\\
    \hline
\end{tabular}
\caption{New APIs for latency-sensitive edge apps in the modified data store tailored to the needs of latency-sensitive mobile applications.}
\label{tab:api_in_edge_store}
}
\hfill
\parbox{.52\columnwidth}{
\centering
\begin{tabular}[\columnwidth]{| c| c |} 
    \hline
    NF & \textbf{New APIs for Application Function}\\
    \hline
    AMF & \textit{Set\_Priority (IpAddress, priority)}\\
    \hline
    AMF & \textit{Revert\_Priority (IpAddress)}\\
    \hline
    RAN & \textit{Set\_Priority (RAN UE NG-AP ID, priority)}\\
    \hline
    RAN & \textit{Revert\_Priority (RAN UE NG-AP ID)}\\
    \hline
\end{tabular}
\caption{New APIs available in \Name for an AF to influence control plane operations at the RAN and AMF.}
\label{tab:api_for_app_influence_on_cpf}
}
\vspace{-0.4in}
\end{table}


\subsection{App-Aware Control Plane Processing}
\label{sec:app_impact_on_control_plane}
In this section, we discuss how an AMF can differentiate between different types of UEs. We also describe how an AMF leverages this information to perform priority processing for the UEs running a latency-sensitive app session.

\noindent{\textbf{5G Services Classes:}} 5G networks are aiming to support three broad classes of services, (i) enhanced Mobile Broad Band (eMBB), (ii) Ultra-Reliable and Low Latency Communication (URLLC), and (iii) delay-tolerant low-complexity Massive IoT (MIoT) \cite{3gpp_architecture, latency_nbiot_catm, iot_in_5g_era_cisco,critical_iot, 3gpp_evaluation_mmtc}.

\noindent{\textbf{UE Classes at AMF:}}
 An AMF can differentiate between the low-complexity (MIoT) and other (eMBB \& URLLC) devices from the information provided by RAN or UE.\footnote{UE context at AMF (table 5.2.2.2.2-1 of the 3GPP document~\cite{3gpp_23_502}) contains information if a UE is a low-complexity device such NB-IoT, LTE-M or RedCap (reduced capability device). Section 1.8 of the 3GPP document~\cite{3gpp_124_008_nas_low_priority_info} suggests a UE can explicitly inform the core network that it is a low-priority device.} An AF, on behalf of app~\cite{mec_in_5g}, can inform which eMBB or URLLC device is to be treated normally or with high priority by the control plane. 
In the context of delay tolerance, our modified AMF can differentiate between the following classes of UEs:


\begin{enumerate}[leftmargin=*]
    \item {\lowPriorityIot:} These are delay-tolerant low-complexity devices such as those used for smart cities, e.g., smart meters. A delay of up to 10\,s is acceptable for these UEs \cite{latency_nbiot_catm, iot_in_5g_era_cisco, 3gpp_evaluation_mmtc}. \Name's AMF is configured to have \textit{lowest priority} for such UEs.
    \item {\mediumPriorityIot:} 
    Includes the rest of devices not included in \lowPriorityIot, such as eMBB and URLLC.
    Such UEs are typically used in agriculture, education, media production, etc \cite{iot_in_5g_era_cisco, cellular_iot_ericsson}. Voice services can also be included in this class of UEs. These UEs have \textit{medium priority} in \Name. 
    \item {\highPriorityIot:} These are devices from the \mediumPriorityIot having an active latency-sensitive data session with an edge app. These UEs have deadlines in the order of few ms \cite{critical_iot, iot_in_5g_era_cisco}. Autonomous vehicles \cite{self_driving_cars_lin2018architectural} and VR headsets \cite{vr-latency} are key examples of such UEs. A UE is only added to this class when an eMBB or URLLC device starts a latency-sensitive data session with an edge app. These UEs have \textit{highest priority} in \Name.
\end{enumerate}



\noindent\textbf{{Priority Processing for Latency-Sensitive Apps:}}
We leverage the UE class information at the AMF to perform priority processing for latency-sensitive apps at RAN and AMF. Radio Resource Control (RRC) layer~\cite{3gpp_architecture} provides a control plane signaling protocol between a UE and RAN. We maintain three separate priority queues for the RRC messages at the BS. The Next Generation Application Protocol (NG-AP) provides the control plane signaling protocol between the RAN and AMF. We maintain three priority queues at the BS for the NG-AP messages from the AMF. Similarly, we maintain three queues at the AMF from the control messages received from the BS. UEs at the RAN and AMF are identified with their unique IDs, \textit{RAN UE NGAP ID} and \textit{AMF UE NGAP ID}, respectively.
 The priority levels are configurable in our design and can be updated by network operators based on their preferences.\footnote{The control processing threads at the BS and AMF by default process 6/10, 3/10, and 1/10 control messages from \highPriorityIot, \mediumPriorityIot, and \lowPriorityIot queues, respectively.} If a high-priority queue is empty, we process messages from one level lower priority queue. Our design requires no changes at the UE. In section \S\ref{appendix_d}, we provide a detailed discussion of the sequence of steps involved when an edge app calls the APIs in Table~\ref{tab:api_for_app_influence_on_cpf} to prioritize their processing.





==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
% \zafar{We have three types of evaluations: (1) Overall performance improvements for real edge apps like CarMap and EMP, (2) A sort of factor analysis describing the benefits offered by each module, (3) A sort of sensitivity analysis; how does EdgeCat perform as we vary application's dynamic state sizes}
In this section, we show the following:

\begin{enumerate}[leftmargin=*]
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    
    \item \textbf{Improvement in Downtime for Real Edge Apps:} \Name reduces app downtime during an app handover by up to $14\times$ and $15.4\times$ for CarMap and EMP, respectively.
    
    \item \textbf{Impact of Proactive App State Migration:} \Name reduces blocking app state migration time
    by more than $2.5\times$ for both CarMap and EMP.
    
    \item \textbf{Impact of App-Aware Control Plane Processing:} \Name reduces 5G handover completion time by up to 3 orders of magnitude for latency-sensitive apps.
    
    \item \textbf{Comprehensive Apps Coverage:} Our sensitivity analysis using our simulation framework~(\S\ref{sec:implementation}) shows \Name can reduce application downtime for a wide variety of applications.
    % \zafar{Revise the last point}.
\end{enumerate}

% \zafar{Perhaps we should have settings and methodology as a separate subsection}
\subsection{Settings and Methodology}
\label{sec:app_handover_setting_and_methodology}
Our test setup consists of seven servers running Ubuntu 18.04.3 with kernel 4.15.0-74-generic. Each server is a dual-socket with 18 cores per socket, Intel Xeon(R) Gold 5220 CPU @ 2.20\,GHz, and with a total memory of 128\,GB. One server hosts the client app. Two servers are running identical instances of the server app. Both servers are installed with \redis v4.0.9 and \memcache v1.5.6. Three servers host an app-aware cellular control plane. 
One server hosts AF, mobility handler, and target BS predictor module of Figure \ref{fig:system_architecture_diagram}. All the figures showing distributions are repeated ten times.

\subsection{Overall Improvement with Real Apps}
\label{sec:eval:combined_impact}

In this section, we show improvement in app downtime with both proactive application state migration and app-aware control plane processing of \Name. Figure \ref{fig:eval:oveerall_app_downtime} shows app downtime during an app handover for CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}. We use the default configuration for both CarMap and EMP.\footnote{Row 1 of Table~\ref{table:eval:carmap_state_migration_time} and Table~\ref{table:eval:emp_state_migration_time} shows default configuration for CarMap and EMP, respectively.} In Figure \ref{fig:eval:oveerall_app_downtime}, ``Baseline'' represents coordinated but reactive app handover (i.e., representing the coordinated handover as shown in 
Figure \ref{fig:challnges_serialized_ho}b) and ``EdgeCat'' represents the modified application version with our proposed design (Figure \ref{fig:challnges_serialized_ho}d). Figure~\ref{fig:eval:oveerall_app_downtime} shows  $14\times$ and $15.4\times$ improvement in median app downtime for CarMap and EMP, respectively, when using \Name. In the following sections, we highlight the contribution of different modules to the overall improvement in app downtime.


% \begin{figure}[tb]
% \centering
% \begin{minipage}[t]{0.48\linewidth}
% \includegraphics[width=\columnwidth]{figs/motivation_app_downtime.png}
% \vspace{-0.3in}
% \caption{App downtime experienced by latency-sensitive edge apps during mobility.
% \label{fig:app_down_time_motivation}
%     \vspace{-0.15 in}
% \end{minipage} 
% \vspace{-0.15 in}
%     \hfill%
% \begin{minipage}[t]{0.47\linewidth}
%     \includegraphics[width=\linewidth]{figs/motivation_handover_uniform_pct_updated.png}
%     \vspace{-0.3 in}
%     \caption{Handover completion time comparison when apps are served by different 5G cores (5GC).}
%     \label{fig:handover_motivation}
% \end{minipage}%
% \end{figure}

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/overall_downtime_distribution_combined_default_config.png}
\vspace{-0.3in}
\caption{Overall improvement in app downtime during an app handover for CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}.}
\vspace{-0.15in}
\label{fig:eval:oveerall_app_downtime}
\end{figure}


\subsection{Target BS Prediction with Real Traces}
\label{sec:eval:target_BS_prediction}

% \Name's two-step state sync mechanism is based on advanced target BS prediction before a handover. 
Figure~\ref{fig:eval:cdf_target_bs_prediction} shows the earliest time (mobility hint forecast horizon) to predict a target BS with the real 5G/4G radio network traces collected in different mobility scenarios. The figure shows \drivingTestAccuracy, \highSpeedTrainAccuracy and \miscAccuracy true predictions 100\,ms before an actual handover with traces collected during driving~\cite{incp_dataset}, in high-speed trains~\cite{li2020beyond}, and miscellaneous mobility scenarios~\cite{mobile_insight_logs}, respectively. The figure shows that with a 100\,ms mobility hint forecast horizon (said differently, predicting the target BS 100~ms before the handover), on average \averageAccuracy true handover predictions are possible. The percentage of true predictions decreases as the mobility hint forecast horizon increases i.e., it is relatively easier to make true predictions 1~ms ahead of the handover (with more measurements) as compared to 2500~ms. A mobility hint received 100\,ms in advance is enough for the edge apps we tested---both CarMap and EMP require less than 100\,ms to provide zero blocking state migration time with default configurations (row 1 of the table~\ref{table:eval:carmap_state_migration_time} and \ref{table:eval:emp_state_migration_time}). 


We also evaluate the inference time for the target BS prediction pipeline. We calculate inference time when predicting target BS for a batch of 50 and 500 users. The median inference time is 8.7\,ms and 9.5\,ms when target BS prediction is performed for a batch of 50 and 500 users, respectively (\S\ref{sec:appendix_inference_time}).

% Figure~\ref{fig:bs_inference_time}\zafar{(1) This figure does not show the CDF of the inference time, it shows the F-1 score and (2) We should not directly discuss a figure in the appendix} shows CDF of the inference time for target BS prediction. 
% The figure shows 8.7\,ms and 9.5\,ms  median inference time when target BS prediction is performed for a batch of 500 and 5000 users\zafar{Where is batching coming from?}, respectively (\S\ref{sec:appendix_inference_time}).
% \zafar{We still need to add the false positive and false negative analysis}

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/bs_prediction_cdf.png}
\vspace{-0.3in}
\caption{Accuracy of the target BS prediction on three real data sets. The annotated statistics show the accuracy when we predict target base stations at least 100\,ms ahead of the actual handover.}
\vspace{-0.15in}
\label{fig:eval:cdf_target_bs_prediction}
\end{figure}




\subsection{Impact of Proactive State Migration on Real Applications}
\label{sec:state_migration_delay}
In this section, we evaluate the performance of \Name's two-step state synchronization on real edge apps with \redis data store. 



\subsubsection{Improvement in CarMap with \Name}
\label{sec:eval:impact_on_carmap}

In Table \ref{table:eval:carmap_state_migration_time}, we compare the performance of CarMap during an app handover in terms of blocking application state migration time---the time from the start of a 5G handover to the completion of state migration. 
% The blocking application state migration time can also be termed as minimum app downtime.
We compare two versions of CarMap: (i) CarMap Baseline represents existing systems where application state migration starts with a 5G handover and (ii) CarMap with \Name represents the case when the application state is stored in our modified \redis data store and two-step state synchronization is performed. Here the two-step state synchronization is performed with a mobility hint of \mobilityHintWindow that results on average in \averageAccuracy correct target BS predictions (Figure~\ref{fig:eval:cdf_target_bs_prediction}). Table \ref{table:eval:carmap_state_migration_time} shows that with \Name, the application blocking state migration time drops to 0.1\,ms and 50.9\,ms from 70.1\,ms and 147.1\,ms when the application dynamic state varies from 14.3\% to 53.8\%, respectively. 
CarMap gets the benefits of proactive application state migration in \averageAccuracy cases and performs like the baseline in \averageFalsePredictioins cases. 

% In contrast, the existing user-space tool (CRIU~\cite{criu}) and container-based migration provide more than 140\,ms and 1.2\,s median app downtime time, respectively (\S\ref{sec:slow_state_migration}).



\newcommand\tikzmark[2]{%
\tikz[remember picture,overlay] 
\node[inner sep=0pt,outer sep=2pt] (#1){#2};%
}

\newcommand\link[2]{%
\begin{tikzpicture}[remember picture, overlay, >=stealth, shorten >= 1pt]
  \draw[->] (#1.east) to  (#2.west);
\end{tikzpicture}%
}

\begin{table}[ht]
\caption{Improvement in CarMap's average \underline{blocking state migration} time with \Name's modified \redis data store. We vary frame upload interval at the vehicle to experiment with different state sizes.} 
\vspace{-0.1in}
\centering 
\begin{tabular}{c c c c}
\hline\hline 
App State & Dynamic & \multicolumn{2}{c}{State Migration Time (ms)}  \\
\cline{3-4}
Size (MBs) & State (\%) & \multicolumn{1}{c}{Baseline} & \multicolumn{1}{c}{\Name} \\
\hline 
2.3 & 4.1 & \tikzmark{a}{70.1} &  \tikzmark{1}{0.1}  \\ 
4.3 & 47.1 & \tikzmark{b}{125.7} & \tikzmark{2}{31.3}  \\
5.4 & 57.3 & \tikzmark{c}{147.1} & \tikzmark{3}{50.9}  \\
\hline 
\end{tabular}
\link{a}{1}
\link{b}{2}
\link{c}{3}
\label{table:eval:carmap_state_migration_time} 
\end{table}

Figure \ref{fig:eval_carmap_rtt} shows message RTT measured on the vehicle when three app handovers are performed during an experiment. The figure shows $\approx$2$\times$ increase in RTT during an app handover when the vehicle client is served with CarMap Baseline. In contrast, CarMap with \Name does not see any significant change in message RTT during an app handover. This improvement is primarily attributed to the mobility hint-based two-step  state synchronization provided in the modified \redis data store.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/carmap_rrt_time_series_1s_upload_interval.png}
\vspace{-0.3in}
\caption{Improvement in message RTT during an app handover when using CarMap with \Name as compared to CarMap Baseline. Settings row 1 of table~\ref{table:eval:carmap_state_migration_time}.}
\vspace{-0.15in}
\label{fig:eval_carmap_rtt}
\end{figure}


\subsubsection{Improvement in EMP with \Name}
\label{sec:eval:impact_on_emp}
In Table \ref{table:eval:emp_state_migration_time}, we compare the performance of EMP baseline and EMP integrated with the modified \redis data store during an app handover. The table shows that the blocking application state migration time drops to $\approx$ 0~ms when using \Name's modified data store with application state size $\approx$ 0.46\,MBs. EMP with \Name shows 3.2$\times$ and 2.5$\times$ improvement over the baseline with application state size 0.71\,MBs and 0.95\,MBs, respectively. The application state properties depend on the application logic. EMP has a relatively smaller state size as compared to CarMap but provides higher blocking state migration time because all the application state is dynamic. 

Our evaluation also shows more than 3$\times$ improvement in message RTT measured on the vehicle under mobility for EMP when using \Name~(\S\ref{appendix_rtt_emp}).

\begin{table}[ht]
\caption{Improvement in EMP's average blocking state migration time when using \Name's modified data store. We vary frame counts per vehicle at the edge server to experiment with different state sizes.} 
\vspace{-0.1in}
\centering 
\begin{tabular}{c c c c} 
\hline\hline
App State & Dynamic & \multicolumn{2}{c}{State Migration Time (ms)}\\
\cline{3-4}
Size (MBs) & State (\%) & \multicolumn{1}{c}{Baseline} & \multicolumn{1}{c}{\Name}  \\
\hline 
0.46 & 100 & \tikzmark{d}{77} & \tikzmark{4}{0.04}  \\ 
0.71 & 100 & \tikzmark{e}{89} & \tikzmark{5}{28}  \\
0.95 & 100 & \tikzmark{f}{145} & \tikzmark{6}{59} \\
\hline 
\end{tabular}
\link{d}{4}
\link{e}{5}
\link{f}{6}
\label{table:eval:emp_state_migration_time} 
\end{table}


\subsection{State Migration Sensitivity Analysis}
\label{eval:factor_analysis}
In this section, we show the impact of varying mobility hint forecast horizon on blocking state migration time for CarMap. As real applications provide limited options to experiment with different state properties, we also show the impact of varying dynamic state sizes with our simulation framework~(\S\ref{sec:impl_target_bs_prediction}).
%interfaced with \memcache data store.  

\subsubsection{Impact of mobility hint}
\label{sec:eval:impact_of_mobility_hint}
Mobility hint forecast horizon varies across handovers (as shown in Figure \ref{fig:eval:cdf_target_bs_prediction}) due to changing radio signal strength. In Figure \ref{fig:migration_time_vs_mobility_hint}, we quantify the impact of different mobility hint forecast horizons on CarMap's 
blocking state migration time. CarMap baseline performs very close to CarMap with \Name when the mobility hint forecast horizon is under 10\,ms. CarMap with \Name performs 3.4$\times$ better than CarMap baseline in median blocking state migration time with a mobility hint forecast horizon of 50\,ms. When mobility hint forecast horizon is larger than 100\,ms, CarMap with \Name provides a median blocking state migration time close to zero as compared to 63\,ms for CarMap baseline. The figure shows that a mobility hint forecast horizon of 100\,ms is enough to provide CarMap zero blocking state migration time.
% \fawad{For all figures, it would help to explain what x and y-axis represent.}

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/carmap_migration_time_vs_mobility_hint.png}
\vspace{-0.2in}
\caption{Impact of varying mobility hint forecast horizon on CarMap's blocking state migration time. Frame upload interval is = 1\,s. Delay budget is $\approx$20\,ms~\cite{ahmad2022idriving_latency_budget}.}
\vspace{-0.2in}
\label{fig:migration_time_vs_mobility_hint}
\end{figure}

\subsubsection{Impact of varying dynamic App state size}
\label{sec:eval:impact_of_dynamic_app_state_
size}

To understand \Name's impact on a variety of applications, we simulate applications having different state properties with our simulation framework. The simulated applications store and perform proactive application state migration with our modified \memcache data store (\S\ref{sec:imp_modified_state_store}). In Figure \ref{fig:migration_time_dynamic_size_impact_memcache}, we compare the blocking state migration time for the simulated application (baseline) and  with \Name. 
% \zafar{Mukhtiar, this is a specific configuration and a natural question is why did you pick this configuration? Why is it representative?}. 
We vary the application dynamic state from 20\% to 100\% with a total state size of 3\,MBs (the observed dynamic state size for real edge apps~, as shown in table~\ref{table:eval:carmap_state_migration_time} \& \ref{table:eval:emp_state_migration_time}). We set the update rate of every dynamic state object to 50 updates/s to simulate high-frequency updates~\cite{zhang2017towards_online_game_updates_rate}.
With 20\% dynamic state, \Name performs 2.5$\times$ better in median blocking state migration time as compared to the baseline. The improvement of \Name over the baseline reduces as the dynamic state percentage increases. With a 100\% dynamic state, the performance of \Name is very close to the baseline. In summary, \Name either reduces the blocking state migration time or performs similarly to the baseline depending on the percentage of dynamic state. 


\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/memcache_dynamic_state_size_impact_migration_time.png}
\vspace{-0.22in}
\caption{\Name's application downtime with varying dynamic state size. The dynamic state update rate = 50 updates/s.}
\vspace{-0.2in}
\label{fig:migration_time_dynamic_size_impact_memcache}
\end{figure}
%when using \memcache data store

\begin{comment}

\subsubsection{Generic App State}
\label{sec:generic_application_state}

In order to simulate a variety of App use cases \cite{?}, Table \ref{table:app_state_time_series} shows seven different state variables having different sizes and update frequencies. The Table shows the user state maintained at the server side of App for every user. We assume no shared state among the users for simplicity. Our simulation setup can be configured to test a variety of App use cases such as Apps having different state sizes (a subset of the dynamic keys) and different update frequencies (static or dynamic with given update frequency). Key 1 in the table represents highly dynamic App state with up to 100 updates/s. Key 1 contains message ID generated at the client, time of the message generation, messages counter for the client at server App and time of message counter increment. The rest of keys can either be configured dynamic (with frequency given in the Table) or static. In our setup, keys 2-7 are dummy App data and random changes are performed on update request in these keys to simulate dynamic state.

\begin{table}[ht]
\caption{User context and update frequency used for simulation. The App state size \cite{ahmad2020carmap} and update frequencies \cite{zhang2017towards_online_game_updates_rate} are representative of latency-sensitive edge Apps.} % title of Table
\centering % used for centering table
\begin{tabular}{c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Variable (Key) \# & Size (Bytes) & Update Frequency \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
1 & 137 & 100 \\ 
2 & 5,120 & 9 or static \\
3 & 5,120 & 4 or static \\
4 & 51,200 & 2 or static \\
5 & 51,200 & 1.6 or static \\
6 & 1,047,522 & 1.42 or static \\
7 & 1,047,522 & 1.25 or static \\
\hline %inserts single line
\end{tabular}
\label{table:app_state_time_series} % is used to refer this table in the text
\end{table}


\subsubsection{Baselines}~\\
\label{sec:app_handover_baselines}
In this section we discuss the following two systems.

\noindent\textbf{\storeDefault:}
For \redis, \storeDefault represents the state migration performed by migrate API available in \redis \cite{reids_migrate_api}. For \memcache, there is no migrate API available by default. We implement it just like implemented in the \redis in following three steps: (i) copy state from local store, (ii) transport state to the target host, and (iii) finally save state in the target store.

\noindent\textbf{\storeNew:} It represents our design (\S\ref{sec:edge_store_for_apps}) based on two-steps synchronization. We implement it in both \redis and \memcache.


\noindent\textbf{Simulation setup:} Every experiment is performed for 2 minutes. UE performs three handovers, each at 30\,s, 60\,s, and 90\,s mark respectively. Handover timings are highlighted with yellow vertical strips in all the figures. For every experiment, client message sending timeout (T) and the number of dynamic keys (given Table \ref{table:app_state_time_series}) is mentioned in the caption. By default, the background state synchronization starts \textcolor{red}{500\,ms} before the actual handover starts.

Figure \ref{fig:migration_time_combined} shows a comparison of user state migration time for both \storeNew and \storeDefault mechanisms when the App dynamic state varies from 1\% to 100\%. The state migration time determines the minimum App-down time which depends on the size of state needs to be migrated after the source App is frozen and before the target server App can serve the user. Figure \ref{fig:migration_time_combined} (top) shows \storeNew reduces App median state migration time by more than \minAppDownTimeRedis for \redis. Similarly, for \memcache in Figure \ref{fig:migration_time_combined} (bottom), the \storeNew reduces the median App state migration time by more than \minAppDownTimeMemcache. The improvement in median App  state migration time even for 100\% dynamic state is because when the server App is updating a key, the background sync mechanism is able to migrate other keys. For both stores, the improvement is attributed to proactive state synchronization of less dynamic state.





% \subsection{Handover impact on the application performance due to state migration}
% \label{sec:impact_of_state_migration}

\subsubsection{Latency improvement in \redis store}~\\
\label{sec:impact_of_state_migration_redis}
In this section we show the improvement of \redisTwoSteps as compared to \redisDefault during App handover.

Figure \ref{fig:redis_app_rtt_less_dynamic}a shows a comparison of packet RTT for \redisTwoSteps and \redisDefault when the server App has < 1\% dynamic state for a user. Figure shows that packet RTT is same for both \redisTwoSteps and \redisDefault when no \handover is taking place. During a \handover, packet RTT for \redisTwoSteps is up to \redisKeyOneRttUptoFactor lower as compared to \redisDefault. Figure \ref{fig:redis_app_rtt_less_dynamic}b shows CDF on the packet RTT during the App handover (yellow highlighted regions in Figure \ref{fig:redis_app_rtt_less_dynamic}a). Figure shows \redisKeyOnePercentile reduction in tail latency (\percentile) during App \handover. These improvements in Figure \ref{fig:redis_app_rtt_less_dynamic} are due to \redisTwoSteps is able to migrate most of the static or less dynamic state in advance and as a result the App downtime due to start migration is significantly reduced.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/redis_less_dynamic.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with < 1\% dynamic state (key 1 in Table~\ref{table:app_state_time_series}) and T = 10\,ms.}
\vspace{-0.1in}
\label{fig:redis_app_rtt_less_dynamic}
\end{figure}

Figure \ref{fig:redis_app_rtt_medium_dynamic} shows packet RTT comparison for \redisTwoSteps and \redisDefault when the server App has $\approx$ 5\% dynamic state for a user. Figure shows up to \redisKeyFourRttUptoFactor and \redisKeyFourPercentile improvement in packet RTT (Figure \ref{fig:redis_app_rtt_medium_dynamic}a) and tail latency (\percentile in Figure \ref{fig:redis_app_rtt_medium_dynamic}b) respectively. These improvements are due to two-steps state synchronization in \redis.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/redis_medium_dynamic.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with $\approx$ 50\% dynamic state (keys 1-4 in Table~\ref{table:app_state_time_series}) and T = 10\,ms.}
\vspace{-0.1in}
\label{fig:redis_app_rtt_medium_dynamic}
\end{figure}

Figure \ref{fig:redis_app_rtt_all_dynamic} shows packet RTT comparison for \redisTwoSteps and \redisDefault when server App is holding 100\% dynamic state for a user. Figure shows up to \redisKeySevenRttUptoFactor and \redisKeySevenPercentile reduction in packet RTT (Figure  \ref{fig:redis_app_rtt_all_dynamic}a) and tail latency (\percentile in Figure \ref{fig:redis_app_rtt_all_dynamic}b) respectively. Here reason for good performance of \redisTwoSteps is that background state migration mechanism  significantly reduces App down-time. 

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/redis_all_dynamic.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with 100\% dynamic state (keys 1-7 in Table~\ref{table:app_state_time_series}) and T = 20\,ms.}
\vspace{-0.1in}
\label{fig:redis_app_rtt_all_dynamic}
\end{figure}



Figure \ref{fig:redis_migrate_vs_background_sync} show a comparison of packet RTT for \redisTwoSteps steps when using the "migrate" API \cite{reids_migrate_api} and our background sync mechanism. Since the "migrate" API blocks the client until the migration is complete, we see significant increase in message RTT when proactive state synchronization is performed. Figure shows 146$\times$ and 29$\times$ increases in message RTT (Figure \ref{fig:redis_migrate_vs_background_sync}a) and tail latency (\percentile in Figure \ref{fig:redis_migrate_vs_background_sync}b) when \redis "migrate" API is used. This performance degradation when using proactive state migration with the \redis "migrate" API is primarily due to the API blocks the client when migrating the user state. 

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/redis_migrate_vs_background_sync.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with $\approx$ 50\% dynamic state (keys 1-4 in Table~\ref{table:app_state_time_series}) and T = 10\,ms.}
\vspace{-0.1in}
\label{fig:redis_migrate_vs_background_sync}
\end{figure}

To summarize, in \cref{fig:redis_app_rtt_less_dynamic,fig:redis_app_rtt_medium_dynamic,fig:redis_app_rtt_all_dynamic} representing different dynamic state scenarios, the \redisTwoSteps performs better than the \redisDefault.

\subsubsection{Latency improvement in \memcache store}~\\
\label{sec:impact_of_state_migration_memcache}
In this section we show the improvement of \memcacheTwoSteps as compared to \memcacheDefault during App handover.

Figure \ref{fig:memcache_app_rtt_less_dynamic} shows packet RTT comparison for \memcacheTwoSteps and \memcacheDefault when the server App has < 1\% dynamic state for a user. Figure shows up to \memcacheKeyFourRttUptoFactor and \memcacheKeyFourPercentile improvement in packet RTT (Figure \ref{fig:memcache_app_rtt_less_dynamic}a) and tail latency (\percentile in Figure \ref{fig:memcache_app_rtt_less_dynamic}b) respectively. These improvements are due to two-steps state synchronization in \memcache.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/memcache_less_dynamic.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with < 1\% dynamic state (key 1 in Table~\ref{table:app_state_time_series}) and T = 10\,ms.}
\vspace{-0.1in}
\label{fig:memcache_app_rtt_less_dynamic}
\end{figure}


Figure \ref{fig:memcache_app_rtt_medium_dynamic} shows packet RTT comparison for \memcacheTwoSteps and \memcacheDefault when the server App has $\approx$ 5\% dynamic state for a user. Figure shows up to \memcacheKeyFourRttUptoFactor and \memcacheKeyFourPercentile improvement in packet RTT (Figure \ref{fig:memcache_app_rtt_medium_dynamic}a) and tail latency (\percentile in Figure \ref{fig:memcache_app_rtt_medium_dynamic}b) respectively.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/memcache_medium_dynamic.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with $\approx$ 50\% dynamic state (keys 1-4 in Table~\ref{table:app_state_time_series}) and T = 10\,ms.}
\vspace{-0.1in}
\label{fig:memcache_app_rtt_medium_dynamic}
\end{figure}

Figure \ref{fig:memcache_app_rtt_all_dynaic} shows packet RTT comparison for \memcacheTwoSteps and \memcacheDefault when the server App has 100\% dynamic state for a user. Figure shows up to \memcacheKeySevenRttUptoFactor and \memcacheKeySevenPercentile improvement in packet RTT (Figure \ref{fig:memcache_app_rtt_all_dynaic}a) and tail latency (\percentile in Figure \ref{fig:memcache_app_rtt_all_dynaic}b) respectively.

\begin{figure}[]
\centering
\includegraphics[width=\columnwidth]{figs/memcache_all_dynamic.png}
\vspace{-0.3in}
\caption{App \handover impact on message RTT with 100\% dynamic state (keys 1-7 in Table~\ref{table:app_state_time_series}) and T = 20\,ms.}
\vspace{-0.1in}
\label{fig:memcache_app_rtt_all_dynaic}
\end{figure}

To summarize, in \cref{fig:memcache_app_rtt_less_dynamic,fig:memcache_app_rtt_medium_dynamic, fig:memcache_app_rtt_all_dynaic} representing different dynamic state scenarios, the \memcacheTwoSteps performs better than the \memcacheDefault.
\end{comment}

\subsection{App-Aware Control Plane Impact}
% \fawad{After the end-to-end experiment, this section and those after it would help articulate how different components of \Name are helping you do so well in the experiment you described above.}
% this section and those after it are looking at some component/s of \Name}
\label{sec:app_aware_control_plane_processing}

We compare the performance of \Name with \Old as a baseline in terms of application performance and handover completion time. Our evaluation of \Old is based on a recently proposed 5G control plane~\cite{neutrino_ton}
% \zafar{say something like a recently proposed 5G control plane}
where the AMF is not aware application running on the UE.




\subsubsection{Impact on app performance}
\label{sec:app_impact_on_app_performance}

To measure the impact of app-aware control plane processing on the application performance, we set up two different  client apps on UE: (i) a CARLA  simulator \cite{carlaPaper, carlaCodeGithub} for autonomous vehicles and (ii) a VR emulator \cite{vr_emulator}. Both of these applications offload processing to an edge server.
As our goal is to quantify the impact of network delays on applications performance during a \handover, we do not perform any additional processing of the data at the edge; the edge server simply sends a hard-coded response to these  applications as soon as input data is received. On the client side, we calculate the percentage of responses that miss the app-specific deadline.

% We perform experiments for 5 minutes while the client is subjected to a \handover every 25\,s on average.


\begin{table}[ht]
\caption{The \% of missed deadlines for latency-sensitive apps during a handover by \Old which drops to zero with \Name. Lower \% is better.}
\vspace{-0.1in}
\centering % used for centering table
\begin{tabular}{l c c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Load (control procedures/sec.) & 20K & 25K & 30K & 35K \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
Autonomous vehicle & 9\% & 25\% & 43\% & 62\% \\ 
VR headset & 13\% & 29\% & 47\% & 66\% \\
\hline %inserts single line
\end{tabular}
\label{table:control_plane_impact_on_apps} % is used to refer this table in the text
\end{table}

Table \ref{table:control_plane_impact_on_apps} shows the percentage of responses that missed the app-specific deadlines when served by \Old. The table shows results when the cellular control plane is serving 60\% of low-priority apps (\lowPriorityIot), 28\% for medium-priority apps (\mediumPriorityIot), and 12\% for high-priority apps (\highPriorityIot), as projected in \cite{iot_traffic_distribution}.


% The table shows results in different load scenarios; where load represents one or more VR or autonomous vehicles and various other devices such as mobile phones and IoT.

Autonomous vehicles have a network delay budget of $\approx$20\,ms~\cite{ahmad2022idriving_latency_budget} to take driving decisions. Table \ref{table:control_plane_impact_on_apps} shows that for an autonomous vehicle, the percentage of missed deadlines increases from 9\% to 62\% as the load increases from 20K to 35K for \Old. When the same App is configured as a high-priority latency-sensitive app (\highPriorityIot ) in \Name, the percentage of missed deadlines drops to zero in all load scenarios.


VR headset-based apps require a latency <16\,ms \cite{delay_impact_on_vr3, delay_impact_on_vr2} to achieve an immersive experience. Table \ref{table:control_plane_impact_on_apps} shows that for a VR app, the percentage of missed deadlines increases from 13\% to 66\% as the load increases from 20K to 35K in \Old. When the same app is configured as a high-priority latency-sensitive app (\highPriorityIot) in \Name, the percentage of missed deadlines drops to zero in all load scenarios which suggests a significant improvement. 

% For both applications, the improvement is due to the app-aware \handover for \highPriorityIot.
The performance gain for edge apps in Table~\ref{table:control_plane_impact_on_apps} is due to a significant reduction in \handover completion time when latency-sensitive apps are configured as \highPriorityIot in \Name. Our evaluation~(\S\ref{sec:appendix_control_plan_bursty_traffic}) shows more than two orders of magnitude reduction in \handover completion time for latency-sensitive apps.







==> evaluation_v1.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we show the following:

\begin{enumerate}[leftmargin=*]
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    
    \item \textbf{Improvement in Downtime for Real Edge Apps:} \Name reduces app downtime during an app handover by up to $14\times$ and $15.4\times$ for CarMap and EMP, respectively.
    
    \item \textbf{Impact of Proactive App State Migration:} \Name reduces blocking app state migration time
    by more than $2.5\times$ for both CarMap and EMP.
    
    \item \textbf{Impact of App-Aware Control Plane Processing:} \Name reduces 5G handover completion time by up to 3 orders of magnitude for latency-sensitive apps.
    
    \item \textbf{Comprehensive Apps Coverage:} Our sensitivity analysis using our simulation framework~(\S\ref{sec:implementation}) shows \Name can reduce application downtime for a wide variety of applications.
    % \zafar{Revise the last point}.
\end{enumerate}

% \zafar{Perhaps we should have settings and methodology as a separate subsection}
\subsection{Settings and Methodology}
\label{sec:app_handover_setting_and_methodology}
\textcolor{blue}{
To evaluate \Name, we created a testbed, as shown in Figure~\ref{fig:eval:testbed}. Our testbed consists of six servers running Ubuntu 18.04.3 with kernel 4.15.0-74-generic and one laptop running Ubuntu 20.04 LTS. Each server is a dual-socket with 18 cores per socket, Intel Xeon(R) Gold 5220 CPU @ 2.20\,GHz, and with a total memory of 128\,GB. The laptop has 20\,GB RAM, 512\,GB SSD, and a GeForce GTX 1060 6\,GB GPU. The laptop hosts the client app. Two servers are running identical instances of the server app. Both servers are installed with \redis v4.0.9 and \memcache v1.5.6. Two servers host an app-aware cellular control plane. 
Two servers host AF, mobility handler, and target BS predictor module of Figure \ref{fig:system_architecture_diagram}. All the figures showing distributions are repeated at least ten times.}

\begin{figure}[]
\centering
\includegraphics[width=0.95\columnwidth]{figs/testbed_updated.png}
\vspace{-0.15in}
\caption{\textcolor{blue}{Testbed for experiments.}}
\label{fig:eval:testbed}
\vspace{-0.2 in}
\end{figure}

\subsection{Overall Improvement with Real Applications}
\label{sec:eval:combined_impact}

In this section, we show improvement in app downtime with both proactive application state migration and app-aware control plane processing of \Name. Figure \ref{fig:eval:oveerall_app_downtime} shows app downtime during an app handover for CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}. We use the default configuration for both CarMap and EMP.\footnote{Row 1 of Table~\ref{table:eval:carmap_state_migration_time} and Table~\ref{table:eval:emp_state_migration_time} shows default configuration for CarMap and EMP, respectively.} In Figure \ref{fig:eval:oveerall_app_downtime}, ``Baseline'' represents coordinated but reactive app handover (i.e., representing the coordinated handover as shown in 
Figure \ref{fig:challnges_serialized_ho}b) and ``EdgeCat'' represents the modified application version with our proposed design (Figure \ref{fig:challnges_serialized_ho}d). Figure~\ref{fig:eval:oveerall_app_downtime} shows  $14\times$ and $15.4\times$ improvement in median app downtime for CarMap and EMP, respectively, when using \Name. In the following sections, we highlight the contribution of different modules to the overall improvement in app downtime.


\begin{figure}[tb]
\centering
\begin{minipage}[t]{0.42\columnwidth}
\includegraphics[width=\columnwidth]{figs/overall_downtime_distribution_combined_default_config.png}
\vspace{-0.35in}
\caption{Overall improvement in app downtime during an app handover for CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}.}
\label{fig:eval:oveerall_app_downtime}
    % \vspace{-0.1 in}
\end{minipage} 
\vspace{-0.15 in}
    \hfill%
\begin{minipage}[t]{0.55\columnwidth}
    \includegraphics[width=\columnwidth]{figs/bs_prediction_cdf.png}
    \vspace{-0.35 in}
    \caption{Accuracy of the early target BS prediction on three real data sets. The annotated statistics show the accuracy of predicting target BS 100 ms ahead of handover.
    }
    % \vspace{-0.1 in}
    \label{fig:eval:cdf_target_bs_prediction}
\end{minipage}%
\end{figure}



\subsection{Target BS Prediction with Real Traces}
\label{sec:eval:target_BS_prediction}

% \Name's two-step state sync mechanism is based on advanced target BS prediction before a handover. 
Figure~\ref{fig:eval:cdf_target_bs_prediction} shows the earliest time to predict a target BS with the real 5G/4G radio network traces collected in different mobility scenarios. The figure shows \drivingTestAccuracy, \highSpeedTrainAccuracy and \miscAccuracy true predictions 100\,ms before an actual handover with traces collected during driving~\cite{incp_dataset}, in high-speed trains~\cite{li2020beyond}, and miscellaneous mobility scenarios~\cite{mobile_insight_logs}, respectively. The figure shows that with a 100\,ms advanced mobility hint (said differently, predicting the target BS 100~ms before the handover), on average \averageAccuracy true handover predictions are possible. The theoretical upper limit of true predictions is \highSpeedTrainMaxAccuracy, \drivingTestMaxAccuracy, and \miscMaxAccuracy in high-speed trains, during driving, and miscellaneous mobility scenarios, respectively. The percentage is computed as the proportion of times when at least one radio sample is received for the true target BS before the handover.
% \zafar{Can we further explain these results: when are unable to predict correctly and what is maximum possible true predictions}
% The percentage of true predictions decreases as the mobility hint forecast horizon increases i.e., it is relatively easier to make true predictions 1~ms ahead of the handover (with more measurements) as compared to 2500~ms\zafar{we can remove this previous statement}. 
A mobility hint received 100\,ms in advance is enough for the edge apps we tested---both CarMap (a localization app) and EMP (a safety app) require less than 100\,ms to provide zero blocking state migration time with default configurations (row 1 of the table~\ref{table:eval:carmap_state_migration_time} \& \ref{table:eval:emp_state_migration_time}). Other safety and localization apps with similar state properties are also expected to perform similarly to CarMap and EMP.
% \zafar{Can we say something about the fact that localization apps like CarMap and car safety apps like EMP will have similar performances?} 


We also evaluate the inference time for the BS prediction pipeline. For a batch of 50 and 500 users, the median inference times are 8.7 ms and 9.5 ms, respectively (\S\ref{sec:appendix_inference_time}).

% We also evaluate the inference time for the  BS prediction pipeline. We calculate inference time when predicting target BS for a batch of 50 and 500 users. The median inference time is 8.7\,ms and 9.5\,ms when target BS prediction is performed for a batch of 50 and 500 users, respectively (\S\ref{sec:appendix_inference_time}).

% We also evaluate the inference time for the  BS prediction pipeline. Our evaluation~(\S\ref{sec:appendix_inference_time}) shows that the per-user median inference time is 285 $\mu$s for a batch size of 50 and 25 $\mu$s for a batch size of 500. This shows a decreasing trend in per-user inference time as the batch size increases.

% \fawad{8.7, and 9.5 to do predictions for all x users? In that case, does it make sense to quantify this as latency per user? That would look more impressive}



\subsection{Impact of Proactive State Migration on Real Applications}
\label{sec:state_migration_delay}
In this section, we evaluate the performance of \Name's two-step state synchronization on real edge apps with \redis data store. 



\subsubsection{Improvement in CarMap with \Name}
\label{sec:eval:impact_on_carmap}

In Table \ref{table:eval:carmap_state_migration_time}, we compare the performance of CarMap during an app handover in terms of blocking application state migration time---the time from the start of a 5G handover to the completion of state migration. 
% The blocking application state migration time can also be termed as minimum app downtime.
We compare two versions of CarMap: (i) CarMap Baseline represents existing systems where application state migration starts with a 5G handover and (ii) CarMap with \Name represents the case when the application state is stored in our modified \redis data store and two-step state synchronization is performed. Here the two-step state synchronization is performed with a mobility hint of \mobilityHintWindow that results on average in \averageAccuracy correct target BS predictions (Figure~\ref{fig:eval:cdf_target_bs_prediction}). Table \ref{table:eval:carmap_state_migration_time} shows that with \Name, the application blocking state migration time drops to 0.1\,ms and 50.9\,ms from 70.1\,ms and 147.1\,ms when the application dynamic state varies from 14.3\% to 53.8\%, respectively. 
CarMap gets the benefits of proactive application state migration in \averageAccuracy cases and performs like the baseline in 3\% cases. 

\newcommand\tikzmark[2]{%
\tikz[remember picture,overlay] 
\node[inner sep=0pt,outer sep=2pt] (#1){#2};%
}

\newcommand\link[2]{%
\begin{tikzpicture}[remember picture, overlay, >=stealth, shorten >= 1pt]
  \draw[->] (#1.east) to  (#2.west);
\end{tikzpicture}%
}


\begin{table}
\parbox{0.48\columnwidth}{
\centering
\begin{tabular}{c c c c}
\hline\hline 
App State & Dynamic & \multicolumn{2}{c}{Migration Time (ms)}  \\
\cline{3-4}
Size (MBs) & State (\%) & \multicolumn{1}{c}{Baseline} & \multicolumn{1}{c}{\Name} \\
\hline 
2.3 & 4.1 & \tikzmark{a}{70.1} &  \tikzmark{1}{0.1}  \\ 
4.3 & 47.1 & \tikzmark{b}{125.7} & \tikzmark{2}{31.3}  \\
5.4 & 57.3 & \tikzmark{c}{147.1} & \tikzmark{3}{50.9}  \\
\hline 
\end{tabular}
\link{a}{1}
\link{b}{2}
\link{c}{3}
\caption{Improvement in CarMap's average \underline{blocking state migration} time with \Name's modified \redis data store. We vary the frame upload interval at the vehicle to experiment with different state sizes.}
\label{table:eval:carmap_state_migration_time} 
}
\hfill
\parbox{.48\columnwidth}{
\centering
\begin{tabular}{c c c c} 
\hline\hline
App State & Dynamic & \multicolumn{2}{c}{Migration Time (ms)}\\
\cline{3-4}
Size (MBs) & State (\%) & \multicolumn{1}{c}{Baseline} & \multicolumn{1}{c}{\Name}  \\
\hline 
0.46 & 100 & \tikzmark{d}{77} & \tikzmark{4}{0.04}  \\ 
0.71 & 100 & \tikzmark{e}{89} & \tikzmark{5}{28}  \\
0.95 & 100 & \tikzmark{f}{145} & \tikzmark{6}{59} \\
\hline 
\end{tabular}
\link{d}{4}
\link{e}{5}
\link{f}{6}
\caption{Improvement in EMP's average \underline{blocking state migration time} when using \Name's modified data store. We vary frame counts per vehicle at the edge server to experiment with different state sizes.} 
\label{table:eval:emp_state_migration_time} 
}
\vspace{-0.35in}
\end{table}

Figure \ref{fig:eval_carmap_rtt} shows message RTT measured on the vehicle when three app handovers are performed during an experiment. The figure shows $\approx$2$\times$ increase in RTT during an app handover when the vehicle client is served with CarMap Baseline. In contrast, CarMap with \Name does not see any significant change in message RTT during an app handover. This improvement is primarily attributed to the mobility hint-based two-step  state synchronization provided in the modified \redis data store.


\begin{figure}[tb]
\centering
\begin{minipage}[t]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figs/carmap_rrt_time_series_1s_upload_interval.png}
\vspace{-0.3in}
\caption{Improvement in message RTT during an app handover when using CarMap with \Name as compared to CarMap Baseline. Settings row 1 of table~\ref{table:eval:carmap_state_migration_time}.}
\vspace{-0.15in}
\label{fig:eval_carmap_rtt}
\end{minipage} 
% \vspace{-0.15 in}
    \hfill%
\begin{minipage}[t]{0.48\columnwidth}
\includegraphics[width=\columnwidth]{figs/carmap_migration_time_vs_mobility_hint.png}
\vspace{-0.3in}
\caption{Impact of early mobility hint on CarMap's blocking state migration time. Frame upload interval = 1\,s. Delay budget $\approx$20\,ms~\cite{ahmad2022idriving_latency_budget}.}
% \vspace{-0.1in}
\label{fig:migration_time_vs_mobility_hint}
\end{minipage}%
\vspace{-0.15in}
\end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=\columnwidth]{figs/carmap_rrt_time_series_1s_upload_interval.png}
% \vspace{-0.3in}
% \caption{Improvement in message RTT during an app handover when using CarMap with \Name as compared to CarMap Baseline. Settings row 1 of table~\ref{table:eval:carmap_state_migration_time}.}
% \vspace{-0.15in}
% \label{fig:eval_carmap_rtt}
% \end{figure}


\subsubsection{Improvement in EMP with \Name}
\label{sec:eval:impact_on_emp}
In Table \ref{table:eval:emp_state_migration_time}, we compare the performance of EMP baseline and EMP integrated with the modified \redis data store during an app handover. The table shows that the blocking application state migration time drops to $\approx$ 0~ms when using \Name's modified data store with app state size $\approx$ 0.46\,MBs. EMP with \Name shows 3.2$\times$ and 2.5$\times$ improvement over the baseline with app state size 0.71\,MBs and 0.95\,MBs, respectively. The app state properties depend on the application logic. EMP has a relatively smaller state size as compared to CarMap but provides higher blocking state migration time because all the application state is dynamic. 

Our evaluation also shows more than 3$\times$ improvement in message RTT measured on the vehicle under mobility for EMP when using \Name~(further details are provided in \S\ref{appendix_rtt_emp}).


\subsection{State Migration Sensitivity Analysis}
\label{eval:factor_analysis}
In this section, we show the impact of varying mobility hints on blocking state migration time for CarMap. As real apps provide limited options to experiment with different state properties, we also show the impact of varying dynamic state sizes with our simulation framework~(\S\ref{sec:impl_target_bs_prediction}).


\subsubsection{Impact of mobility hint}
\label{sec:eval:impact_of_mobility_hint}
The advanced mobility hint varies across handovers (as shown in Figure \ref{fig:eval:cdf_target_bs_prediction}) due to changing radio signal strength. In Figure \ref{fig:migration_time_vs_mobility_hint}, we quantify the impact of different advanced mobility hints on CarMap's 
blocking state migration time. CarMap baseline performs very close to CarMap with \Name when the advanced mobility hint is under 10\,ms. CarMap with \Name performs 3.4$\times$ better than CarMap baseline in median blocking state migration time with an advanced mobility hint of 50\,ms. When the advanced mobility hint is larger than 100\,ms, CarMap with \Name provides a median blocking state migration time close to zero as compared to 63\,ms for CarMap baseline. The figure shows that an advanced mobility hint of 100\,ms is enough to provide CarMap zero blocking state migration time.


% \begin{figure}[]
% \centering
% \includegraphics[width=\columnwidth]{figs/carmap_migration_time_vs_mobility_hint.png}
% \vspace{-0.2in}
% \caption{Impact of varying mobility hint forecast horizon on CarMap's blocking state migration time. Frame upload interval is = 1\,s. Delay budget is $\approx$20\,ms~\cite{ahmad2022idriving_latency_budget}.}
% \vspace{-0.2in}
% \label{fig:migration_time_vs_mobility_hint}
% \end{figure}

\subsubsection{Impact of varying dynamic App state size}
\label{sec:eval:impact_of_dynamic_app_state_
size}

To understand \Name's impact on a variety of apps, we simulate applications having different state properties with our simulation framework. The simulated apps store and perform proactive app state migration with our modified \memcache data store (\S\ref{sec:imp_modified_state_store}). In Figure \ref{fig:migration_time_dynamic_size_impact_memcache}, we compare the blocking state migration time for the simulated app (baseline) and  with \Name. 
% \zafar{Mukhtiar, this is a specific configuration and a natural question is why did you pick this configuration? Why is it representative?}. 
We vary the app dynamic state from 20\% to 100\% with a total state size of 3\,MBs (the observed dynamic state size for real edge apps~, as shown in table~\ref{table:eval:carmap_state_migration_time} \& \ref{table:eval:emp_state_migration_time}). We set the update rate of every dynamic state object to 50 updates/s to simulate high-frequency updates~\cite{zhang2017towards_online_game_updates_rate}.
With 20\% dynamic state, \Name performs 2.5$\times$ better in median blocking state migration time as compared to the baseline. The improvement of \Name over the baseline reduces as the dynamic state percentage increases. With a 100\% dynamic state, the performance of \Name is very close to the baseline. In summary, \Name either reduces the blocking state migration time or performs similarly to the baseline depending on the percentage of dynamic state. 


% \begin{figure}[]
% \centering
% \includegraphics[width=\columnwidth]{figs/memcache_dynamic_state_size_impact_migration_time.png}
% \vspace{-0.22in}
% \caption{\Name's application downtime with varying dynamic state size. The dynamic state update rate = 50 updates/s.}
% \vspace{-0.2in}
% \label{fig:migration_time_dynamic_size_impact_memcache}
% \end{figure}

\begin{table}
\begin{minipage}{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/memcache_dynamic_state_size_impact_migration_time.png}
\vspace{-0.3in}
\captionof{figure}{\Name's application downtime with varying dynamic state size. The dynamic state update rate = 50 updates/s.}
\vspace{-0.1in}
\label{fig:migration_time_dynamic_size_impact_memcache}
\end{minipage}\hfill
\begin{minipage}{0.45\columnwidth}
\caption{The \% of missed deadlines for latency-sensitive apps, such as VR headset and autonomous vehicle (AV), during a handover by \Old which drops to zero with \Name. Load represents control procedures per second. Lower \% is better.}
\vspace{-0.15in}
\label{table:control_plane_impact_on_apps}
\centering
\begin{tabular}{l c c c c} 
\hline\hline 
Load & 20K & 25K & 30K & 35K \\ [0.5ex] 
\hline
AV & 9\% & 25\% & 43\% & 62\% \\ 
VR headset & 13\% & 29\% & 47\% & 66\% \\
\hline
\end{tabular}
\end{minipage}
\vspace{-0.15in}
\end{table}


\subsection{Application-Aware Control Plane Impact}
\label{sec:app_aware_control_plane_processing}
In this section, we compare the performance of \Name with \Old---a recently proposed 5G control plane~\cite{neutrino_ton}
where the AMF is not aware application running on the UE.


% We compare the performance of \Name with \Old as a baseline in terms of application performance and handover completion time. Our evaluation of \Old is based on a recently proposed 5G control plane~\cite{neutrino_ton}
% where the AMF is not aware application running on the UE.




\subsubsection{Impact on app performance}
\label{sec:app_impact_on_app_performance}

To measure the impact of app-aware control plane processing on the app performance, we set up two different  client apps on UE: (i) a CARLA  simulator \cite{carlaPaper, carlaCodeGithub} for autonomous vehicles and (ii) a VR emulator \cite{vr_emulator}. Both of these apps offload processing to an edge server.
As our goal is to quantify the impact of network delays on applications performance during a \handover, we do not perform any additional processing of the data at the edge; the edge server simply sends a hard-coded response to these  apps as soon as input data is received. We calculate the percentage of responses that miss the app-specific deadline on the client.

% We perform experiments for 5 minutes while the client is subjected to a \handover every 25\,s on average.


% \begin{table}[ht]
% \caption{The \% of missed deadlines for latency-sensitive apps during a handover by \Old which drops to zero with \Name. Lower \% is better.}
% \vspace{-0.1in}
% \centering % used for centering table
% \begin{tabular}{l c c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Load (control procedures/sec.) & 20K & 25K & 30K & 35K \\ [0.5ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% Autonomous vehicle & 9\% & 25\% & 43\% & 62\% \\ 
% VR headset & 13\% & 29\% & 47\% & 66\% \\
% \hline %inserts single line
% \end{tabular}
% \label{table:control_plane_impact_on_apps} % is used to refer this table in the text
% \end{table}

Table \ref{table:control_plane_impact_on_apps} shows the percentage of responses that missed the app-specific deadlines when served by \Old. The table shows results when the cellular control plane is serving 60\% of low-priority apps (\lowPriorityIot), 28\% for medium-priority apps (\mediumPriorityIot), and 12\% for high-priority apps (\highPriorityIot), as projected in \cite{iot_traffic_distribution}.


% The table shows results in different load scenarios; where load represents one or more VR or autonomous vehicles and various other devices such as mobile phones and IoT.

Autonomous vehicles~\cite{ahmad2022idriving_latency_budget} and VR headset-based apps~\cite{delay_impact_on_vr3, delay_impact_on_vr2} have a delay budget of $\approx$20\,ms and <16\,ms, respectively. Table \ref{table:control_plane_impact_on_apps} shows $\approx$ 50\% increase in missed deadlines for both apps as the load increases from 20K to 35K when served with \Old. When the same apps are configured as high-priority latency-sensitive apps (\highPriorityIot ) in \Name, the percentage of missed deadlines drops to zero in all load scenarios.
% Autonomous vehicles have a network delay budget of $\approx$20\,ms~\cite{ahmad2022idriving_latency_budget} to take driving decisions. Table \ref{table:control_plane_impact_on_apps} shows that for an autonomous vehicle, the percentage of missed deadlines increases from 9\% to 62\% as the load increases from 20K to 35K for \Old. When the same app is configured as a high-priority latency-sensitive app (\highPriorityIot ) in \Name, the percentage of missed deadlines drops to zero in all load scenarios.
% VR headset-based apps require a latency <16\,ms \cite{delay_impact_on_vr3, delay_impact_on_vr2} to achieve an immersive experience. Table \ref{table:control_plane_impact_on_apps} shows that for a VR app, the percentage of missed deadlines increases from 13\% to 66\% as the load increases from 20K to 35K in \Old. When the same app is configured as a high-priority latency-sensitive app (\highPriorityIot) in \Name, the percentage of missed deadlines drops to zero in all load scenarios which suggests a significant improvement. 
% For both applications, the improvement is due to the app-aware \handover for \highPriorityIot.
The performance gain for edge apps in Table~\ref{table:control_plane_impact_on_apps} is due to a significant reduction in \handover completion time when latency-sensitive apps are configured as \highPriorityIot in \Name. Our evaluation~(\S\ref{sec:appendix_control_plan_bursty_traffic}) shows more than two orders of magnitude reduction in \handover completion time for latency-sensitive apps.







==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}
A summary of \Name's implementation is given below.

\subsection{Target BS Prediction}
\label{sec:impl_target_bs_prediction}
We implement the LSTM network for the target BS prediction in Python on top of the \textit{Keras version 2.9.0}. The LSTM network has a total of 8 layers and 15,923 trainable parameters. 
% (\S\ref{appendix_lstm_binary_classifier}).
Our data set for training the LSTM network consists of radio network traces collected in high-speed trains~\cite{hst_sigcomm_dataset}, driving tests~\cite{incp_dataset}, and other miscellaneous mobility scenarios~\cite{mobile_insight_logs}. The data set consists of a total of \totalHandovers handover events. The radio traces in the data set are sampled at a $\approx$50\,ms interval.
% (\S\ref{appendix_dataset_description}).

\subsection{Modified External Data Store}
\label{sec:imp_modified_state_store}
We implement all our modifications (as discussed in \S\ref{sec:design_app_state_migration}) in the \redis \cite{redis_store} and \memcache \cite{memcached_store} data stores. We also implement our new APIs in Table \ref{tab:api_in_edge_store} on top of the common client APIs (get, set, delete, etc.) available in these data stores. We implement three versions of the modified \redis data store, each one in C++, Java, and Python on top of the open-source clients \cite{redis_cpp}, \cite{redis_java}, and \cite{redis_python}, respectively. We also implement a Python version of the modified \memcache data store on top of \textit{pymemcache 4.0.0} Python package. We interface our modified data stores with the following apps:

\noindent\textbf{CarMap:} We modify the open-source C++ code-base of CarMap \cite{carmap_gitub, ahmad_carmap} to use the C++ version of our modified \redis data store for application state storage and updates. Our changes to CarMap comprise of $\approx$477 lines of code.  %Our modifications to CarMap comprise six C++ and six C++ header files with $\approx$477 lines of code.

\noindent\textbf{EMP:} We modify the open-source Java code-base of EMP \cite{emp_gitub, zhang2021emp} to use the Java version of our modified \redis data store. Our changes to EMP consist of $\approx$350 lines of code. 

\subsection{Edge Application Simulation Framework}
\label{sec:edge_apps_simulation_framework}
App state properties (i.e., state size,  dynamic state percentage, state update rate) vary across different edge apps. Real edge apps provide limited options to vary these properties and it is not practical to update many edge apps.
Consequently, for comprehensive experimental coverage, we develop a simulation framework in Python. The server side of the framework allows the user to configure the user's application state such as the number of state objects and their properties (sizes, update rates, etc.). The client-side allows the generation of application traffic toward the server and receives responses.
% We also implement all the critical modules for proactive App state migration of figure \ref{fig:system_architecture_diagram} in python for interfacing with the simulation framework. 
The framework interfaces with both modified \redis and \memcache data stores. The simulation framework consists of $\approx$1147 lines of code.



% \subsection{EMP}
% \label{sec:impl_emp}
% We have modified the open-source Java code base of EMP \cite{emp_gitub, zhang2021emp} to use the Java version of our modified edge \redis data store for proactive state migration. The EMP stores the App state in our modified edge data store and performs proactive state migration through the new APIs available in table \ref{tab:api_in_edge_store}. We use timers to trigger mobility hints and mobility handover to perform App state migration. Our changes to the EMP are the addition of 6 new files with $\approx$ 350 lines of code.

% \subsection{CarMap}
% \label{sec:impl_carmap}
% We have modified the open-source C++ code-base of CarMap \cite{carmap_gitub, ahmad_carmap} to use the C++ version of our modified edge \redis data store for proactive App state migration. CarMap stores the App state in our modified edge data store and performs proactive App state migration through the APIs exposed in table \ref{tab:api_in_edge_store}. We use timers to trigger mobility hint and mobility handover to perform proactive App state migration. Our modifications to CarMap comprise 6 C++ and 6 C++ header files with $\approx$ 477 lines of code.

% \subsection{Edge App simulation framework}
% \label{sec:imp_edge_app_emulation_framework}
% State properties vary across different edge Apps and it is not practical to identify the user's App state and modify the source code for several edge Apps developed in different programming languages. To give wider experimental coverage to the modified data stores, we have developed a framework in python language that allows the user to configure the user state such as the number of state variables and their properties (sizes, update rates, etc.). We also implement all the key modules for proactive App state migration of figure \ref{fig:system_architecture_diagram} in python. The edge App simulation framework works with both of the modified edge \redis and \memcache data stores. Our simulation framework has a total of 26 python files and $\approx$ 1147 lines of code.

\subsection{Application-Aware Control Plane Processing}
\label{sec:imp_app_aware_control_plane_processing}
We have modified the open-source C/C++ code-base of a recently proposed cellular control plan~\cite{neutrino_gitub, neutrino_ton} to implement app-aware control plane processing (\S\ref{sec:app_impact_on_control_plane}). 
We implement the RAN-related APIs of Table \ref{tab:api_for_app_influence_on_cpf} in  the control traffic generator (emulating both UE and BS) of \cite{neutrino_gitub}. Similarly, we implement the AMF-related APIs of Table \ref{tab:api_for_app_influence_on_cpf} in the control plane function (AMF + SMF) of \cite{neutrino_gitub}. 
Our changes to \cite{neutrino_gitub} consist of the addition of $\approx$967 lines of code.




==> intro.tex <==
% \vspace{-0.1in}
\section{Introduction}
5G and next-generation cellular networks aim to support emerging latency-sensitive applications (apps), such as safety apps for connected and autonomous vehicles~\cite{ahmad_carmap, zhang2021emp, infra_structure_assisted_car_map}, virtual and augmented reality (AR/VR) \cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}, edge-based video analytics~\cite{killer_app_edge_computing}, and multi-player online gaming \cite{online_gamming_delay_budget,zhang2017towards_online_game_updates_rate}. These applications place new demands of ultra-low latency on the 5G infrastructure, e.g., VR apps with head tracking systems require latency of less than 17ms to achieve perceptual stability~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

To reduce end-to-end delays and enable such applications, 5G networks are integrating Edge Computing~\cite{ar_vr_satyanarayanan2017emergence,mec_in_5g}; a paradigm whereby applications are hosted closer to the users, on cell towers, cell aggregation sites, or other edge sites~\cite{mec_in_5g, etsi2, etsi3}. Many cellular providers are partnering with cloud providers for deploying edge apps inside the cellular infrastructure~\cite{azure_edgezone, aws_wavelength, google_carriers}.  

Hosting applications at the network edge can significantly reduce delays. However, it also makes it challenging to ensure that users always receive low latency as they move across different locations. This in turn requires support to handover clients to different edge sites with negligible delays~\cite{mec_app_mobility_api_021}.
%they change locations with user mobility, it can cause the current edge host to be no longer optimal, requiring App handover~\cite{survey_on_service_migration, fast_service_migratioin_using_vm, efficient_container_migration}. 
These application handovers are likely to be frequent~\cite{frequent_handover_zhou20215g, frequent_migration_abouaomar2021deep,  driving_frequent_app_handoverr,mec_in_5g, mec_evolution_toward_5g_etsi, etsi2} for a significant fraction of 5G use cases as more than 50\% of 5G IoTs are expected to be highly mobile apps related to the automotive industry \cite{5g_edge_computing_aws_53p}.\footnote{5G networks will have 5 billion connected IoTs by 2025~\cite{iot_in_5g_era_cisco}.} 
%A recent 5G measurement study~\cite{narayanan2020first} suggests 30+ app handovers are possible in less than 8 minutes duration when edge Apps are deployed on base stations (BSs).
%Many mobile applications are also stateful\footnote{By stateful we mean the application processing depends on the state previously reported by the client and/or generated at the server.}~\cite{zhang2021emp, ahmad_carmap, zhang2017towards_online_game_updates_rate, shi2019mobile_edge_vr, full_body_tracking_vr} and migrating stateful applications over 5G can cause significant application downtime\footnote{The duration for which an application cannot serve the users.} \cite{vm_container_migration_in_5g_mec,live_migration_yang2021multitier} (\S\ref{sec:slow_app_handover}). 
Many of these edge apps are stateful~\cite{zhang2021emp, ahmad_carmap, zhang2017towards_online_game_updates_rate, shi2019mobile_edge_vr, full_body_tracking_vr} and migrating stateful applications over 5G can cause significant application downtime during mobility~\cite{vm_container_migration_in_5g_mec,live_migration_yang2021multitier} (\S\ref{sec:slow_app_handover}). Consequently, if the application downtime exceeds the delay budget for latency-sensitive apps, it can compromise user safety in the case of connected cars~\cite{zhang2021emp, ahmad_carmap} or cause users motion sickness when using immersive mobile VR~\cite{motion_sickness_kundu2021study}.

%such as compromise on user's safety for CarMap \& EMP and immersive experience for mobile VR.

%by which we mean their  processing depends on the state previously reported by the client and/or generated at the server. %\footnote{Throughout the 
%Migration of stateful applications over 5G can cause significant application downtime\footnote{The duration for which an application cannot serve the users.} during client mobility~\cite{vm_container_migration_in_5g_mec,live_migration_yang2021multitier}.
In this paper, we first step back and ask the question, \textit{what are the key architectural bottlenecks in enabling stateful mobile edge applications over 5G}? We identify three key issues in enabling fast application handovers during mobility (illustrated in Figure~\ref{fig:challnges_serialized_ho}):


%of ms, for latency-sensitive applications~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

%Consequently, application downtime can be several seconds, in contrast to the delay budget of under a few tens of ms, for latency-sensitive applications~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/app_handover_challenges_contributions.png}
\vspace{-0.3in}
\caption{Key issues and possible directions to reduce downtime during app handover due to mobility. 5G handover delays range between 87-170\,ms~\cite{understanding_operational_5g} whereas session migration for edge apps takes atleast 140\,ms with existing techniques~(\S\ref{sec:slow_state_migration}).}
\label{fig:challnges_serialized_ho}
\vspace{-0.15in}
\end{figure}


\begin{itemize}[leftmargin=*]
\item \textbf{Uncoordinated and Reactive App Session Migration:}
A stateful application handover involves two key steps: (i) the user's network session migration (5G handover) and (ii) the user's application session migration.  
%A 4G handover delay is 25\,ms on average (range 14-177\,ms)~\cite{dpcm}
%5G handovers typically range between 87-170\,ms~\cite{hassan2022vivisecting, understanding_operational_5g} whereas session migration for edge apps takes atleast 140\,ms with existing techniques~(\S\ref{sec:slow_state_migration}). 
If the network and application session migration is uncoordinated, this can cause prolonged application downtime (as shown in Figure \ref{fig:challnges_serialized_ho}a). For a coordinated application handover, the decision of \textit{when} 
and \textit{where} (to which target edge host) to perform an application handover depends on the 5G handover decision and target base station (BS) selection, respectively. Figure~\ref{fig:challnges_serialized_ho}b shows that even if we perfectly synchronize the 5G handover and application session migration events, application downtime can still be significantly higher than the delay budgets of latency-sensitive edge apps, which are in the order of 10ms~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}. %The app delay budget is the maximum amount of downtime an application can handle after which its performance degrades. %To reduce application downtimes, we need both a \textit{coordinated} and \textit{proactive} approach in which the target base station can be predicated in advance and shared with edge apps so they can proactively start app state migration, as shown in Figure \ref{fig:challnges_serialized_ho}(c). 
 
 
 %The challenge is that even if the 5G handover and application session migration events are perfectly synchronized, the minimum downtime for an edge app is the maximum delay of 5G handover completion time and application session migration time (Figure \ref{fig:challnges_serialized_ho}(b)). Consequently, application downtime can be significantly higher than the delay budgets of latency-sensitive edge apps, which are in the order of tens of milliseconds~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

\item \textbf{Slow App Session Migration:} A key challenge with speeding up session migration of stateful applications is that they typically require the user's up-to-date app state at the target edge host before a user connects to it~\cite{harchol2018cessna}. However, existing techniques for application session migration are either slow~\cite{live_migration_8000803,vm_container_migration_in_5g_mec, hardware_accelerated_live_migration,efficient_container_migration,live_migration_269357, criu} or they implement app-specific optimizations~\cite{fast_check_point_recovery} which cannot be generalized (\S\ref{sec:slow_state_migration}). A key challenge is to design a session migration technique that is \textit{fast} and \textit{generic}. %A key challenging to design an App state migration technique that is fast and generic across Apps.
%This means if we have the edge application running on the target edge site, we will still have to delay of transferring user's application state. The existing application-agnostic state migration techniques based on containers~\cite{live_migration_8000803,vm_container_migration_in_5g_mec, hardware_accelerated_live_migration,efficient_container_migration,live_migration_269357}, VMs~\cite{fast_service_migratioin_using_vm}, and user space tools such as CRIU~\cite{criu} are slow (i.e., provides several seconds downtime~\S\ref{sec:slow_state_migration}).
%App-specific techniques \cite{fast_check_point_recovery} require the App developer to identify the App dynamic state, track its update rate, and synchronize it with a target App instance which can be a daunting task for an App developer. It is challenging to design an App state migration technique that is fast and generic across Apps.

\item \textbf{App-agnostic 5G Handover:}
We observe that even if we somehow address the issue of slow app session migration, the time required for a 5G handover can become a bottleneck in enabling latency-sensitive edge apps, as shown in Figure~\ref{fig:challnges_serialized_ho}c (\S\ref{sec:app_agnostic_5g_handover}). %This can happen if the 5G control plane is overloaded~\cite{neutrino_ton,  mmlite}  or experiencing faults~\cite{cellclone, echo}. 
An architectural issue is that 5G control plane processing is \textit{application-agnostic} and there are no 5G interfaces through which edge apps can inform the cellular control plane of their latency requirements.

%A 5G handover can become a bottleneck if cellular control plane functions at the edge~\cite{neutrino, iot_in_5g_era_cisco} are experiencing high traffic loads~\cite{neutrino_ton,  mmlite} or faults~\cite{cellclone, echo}. 
% \zafar{It depends -- if app session handover takes longer, it will still be the bottleneck as shown in Figure 1b} \textcolor{red}{I think this point is still valid. I will discuss it.}
%A 5G handover can become a performance bottleneck if control plane functions at the edge~\cite{neutrino, iot_in_5g_era_cisco} are experiencing a high traffic load~\cite{neutrino_ton,  mmlite} or faults~\cite{cellclone, echo}. 
% Prior work deals with control plane faults, such as failures~\cite{echo, neutrino} and stragglers~\cite{cellclone}.
% \zafar{if control plane functions are slow -- this could be due to high load but also due to other reasons (memory issue, more generally hardware faults, software bug etc) which can cause the control plane functions to become stragglers}
%High control plane load is likely in 5G as it aims to support dense deployments, with up to 1 million devices per square km \cite{iot_in_5g_era_cisco}. In addition, an edge-based cellular control plane, having limited resources as compared to cloud-based deployments \cite{trivedi2020sharing, edge_resouces, edge_resources_globe}, may not meet instantaneous control traffic load spikes due to IoT devices generating synchronous control traffic ~\cite{mmtc_sync_traffic_ferdouse2017congestion, mmtc_sync_traffic_laner2015traffic}. An architectural issue is that 5G control plane processing is \textit{application-agnostic} and there no interfaces through which edge apps can inform the control plane of their latency needs.
%A slow 5G handover can become a performance bottleneck in performing a fast App handover as depicted in Figure~\ref{fig:challnges_serialized_ho}(c).

\end{itemize}

To address the above issues, we propose a new system architecture, \Name (\underline{EdgeCat}alyst), for edge apps over 5G. \Name is a cross-layer design that (a) leverages the interfaces exposed by the Multi-access Edge Computing (MEC) framework in 5G~\cite{mec_in_5g} to share radio network information with edge apps so they can proactively perform application state migration, and (b) proposes new interfaces to share application's latency requirements with the 5G control plane for speeding up 5G handovers. \Name consists of the following key ideas:
%\Name leverages the radio network information~\cite{5g_mec_rni1} exposed by Multi-access Edge Computing MEC~\cite{mec_in_5g} in 5G to speed up App session migration. In addition, it leverages application-level information to speed up 5G handover. Following are the key ideas in \Name.
% Handover prediction~\cite{hassan2022vivisecting} is relatively easy as it involves the user's network session migration from a source to any neighboring BS. Intuitively, a handover can be expected when signal strength shows decreasing trend for a source BS and an increasing trend for any of the neighboring BSs.  In contrast, a target BS prediction requires advanced forecasting of the correct target BS out of multiple neighboring BSs.
%A challenge here is to predict the target BS with reasonable accuracy before the 5G handover to enable proactive App session migration.



\begin{itemize}[leftmargin=*]
    
\item \textbf{Target BS Prediction:} To reduce app downtimes, we need both a \textit{coordinated} and \textit{proactive}  approach to application handovers. To enable such an approach, \Name predicts the target base station of a 5G handover event in advance so edge apps can proactively start app state migration, as shown in Figure \ref{fig:challnges_serialized_ho}c. We observe that the problem of predicting when a 5G handover occurs is different from predicting the actual target base station. While 5G handovers are relatively easier to predict~\cite{hassan2022vivisecting}, target base station prediction can be harder as it generally involves multiple candidate base stations~(\S\ref{sec:challenges:reactive_app_session_migration}). To make target base predictions, we design a model based on a Long Short Term Memory (LSTM) neural network. It uses the data exposed by the Radio Network Information (RNI) API in MEC~\cite{5g_mec_rni1} (\S\ref{sec:design:target_bs_predction}), which consists of radio information about mobile clients to edge apps. We train and test our model on multiple real 5G/4G radio network traces, including those collected during driving tests~\cite{incp_dataset}, high-speed trains~\cite{li2020beyond}, and other miscellaneous mobility scenarios \cite{mobile_insight_logs}. Our model on average correctly predicts \averageAccuracy of the target BSs
100\,ms ahead of an actual handover~(\S\ref{sec:eval:target_BS_prediction}). We refer to this advanced target base prediction as a \textit{mobility hint} for apps.% We call the advanced mobility prediction a mobility hint % This advance knowledge of target base stations can be used by edge apps to proactively start app migration. %This has the potential of reducing app down time due to proactive state, while incurring no additional overheads in case of false positives 




%leverages most up-to-date user mobility-related information available in the radio signal strength measurements reported by the user equipment (UE) to the BS.
%The most up-to-date user mobility-related information is available in the radio signal strength measurements reported by the user equipment (UE) to the BS. 
%The MEC in 5G exposes this information to the edge apps through the radio network information (RNI~\cite{5g_mec_rni1}) APIs. %to optimize its performance \cite{mec_in_5g}. 
%We leverage the RNI APIs to predict the target BS before an actual network handover starts. For this purpose, we design an LSTM-based neural network and train it on control plane traces collected in high-speed trains \cite{li2020beyond}, driving tests \cite{incp_dataset} and other miscellaneous mobility scenarios \cite{mobile_insight_logs}. 
% \zafar{How would training happen in practice? I imagine any operator can dynamically train the model for their datasets and can update the model as more data is received. We need to separate how training will be done in a real telecom network vs. the training data sets that we have used in this paper to show the efficacy of the model}
%We call the advanced mobility prediction a mobility hint. \Name uses the mobility hint to perform proactive App state migration. %A true BS prediction can significantly reduce App state migration time while a false prediction causes no degradation in performance.

\item \textbf{Two-Step App State Synchronization:}
An application can proactively synchronize all or a subset of the user's app state with the target edge host based on the mobility hint. However, proactively synchronizing a highly dynamic state object (i.e., state object that is frequently updated) has little advantage, as it may soon become stale. In addition, it is a daunting task for developers to identify and track different types of state objects to determine which subset of the state to proactively synchronize. We instead propose extending existing data stores (e.g., \redis \cite{redis_store} and \memcache \cite{memcached_store}) to store and track the state of an edge app. %ask the developer to store state variables in our modified data stores (\redis \cite{redis_store} and \memcache \cite{memcached_store}). 
Specifically, we extend existing data stores to track the update rate for every state object for an edge app (\S\ref{sec:design_app_state_migration}). 
In addition, we expose new APIs to edge apps (Table~\ref{tab:api_in_edge_store}) to synchronize the state objects that have low update rates on receiving a mobility hint and synchronize the rest of the dynamic app state when a 5G handover starts. This reduces the blocking time during state migration, which in turn reduces the app downtime (\S\ref{sec:state_migration_delay}).
%Our modified state store offloads the dynamic state tracking and two-step app state synchronization from apps (\S\ref{sec:design_app_state_migration}).


\item \textbf{App-Aware Control Plane Processing:}
To make 5G control plane processing application-aware, we introduce new APIs (Table \ref{tab:api_for_app_influence_on_cpf}) in the 5G control plane to allow the edge apps to report their latency requirements and prioritize their control plane processing accordingly (\S\ref{sec:app_impact_on_control_plane}). The server side of the latency-sensitive app calls these APIs through the MEC \cite{mec_in_5g} to influence their control plane processing. The reason for only allowing the server side of the app to call these APIs because it is either directly in network operator control or managed by third parties in collaboration with the network operator and as a result, it is a more suitable place to avoid misuse of these APIs, in contrast to clients. Our experiments show that an app-aware 5G control plane can result in a substantial reduction in 5G handover delays, which can help in bringing the downtime of edge apps within their delay budgets~(\S\ref{sec:app_aware_control_plane_processing}).

%Figure~\ref{fig:challnges_serialized_ho}(c) shows a 5G handover can be a key bottleneck to reduce App downtime. Figure~\ref{fig:challnges_serialized_ho}(d) shows a significant reduction in App downtime with an App-aware 5G control plane.
\end{itemize}
% to support faster application handover for latency-sensitive edge apps in 5G
To show the efficacy of the above ideas, we implement \Name. We implement the target BS prediction module using an 8-layer LSTM neural network on top of the Keras library~\cite{keras_library}. Our data sets consist of \totalHandovers handovers. On the application layer, we implement dynamic state tracking and two-step state synchronization in \redis~\cite{redis_store} and \memcache~\cite{memcached_store} data stores~(\S\ref{sec:design_app_state_migration}). To evaluate the impact of \Name on real edge apps, we modify two recent open-source edge apps, CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}, to use our modified \redis data store for proactive state synchronization. As real applications provide limited options to vary app state properties (e.g., state sizes, update rate, etc.), we implement a simulation framework in Python to simulate the behavior of a wide variety of latency-sensitive edge apps~(\S\ref{sec:imp_modified_state_store}). We interface a Python version of both modified \memcache and \redis key-value data stores with the simulation framework to evaluate the impact of two-step state syncing on a wide variety of application behaviors. To implement app-aware control plane processing, we modify a recently proposed cellular control plane~\cite{neutrino_ton}. We provide further details of our implementations in \S\ref{sec:implementation}. We open-source our code on an anonymous Github link: \href{\repourl}{\repourl}.

Our evaluation shows up to $14\times$ and $15.4\times$ improvement in app downtime for CarMap and EMP, respectively. \Name on average correctly predicts \averageAccuracy of the target BSs 100\,ms ahead of an actual handover (\S\ref{sec:eval:impact_of_mobility_hint}). Consequently, CarMap and EMP show more than $3\times$ and $2.5\times$ improvement in application state migration time, respectively~(\S\ref{sec:state_migration_delay}). 
% \Name significantly improves application state migration time in \averageAccuracy cases with correct BSs predictions or performs similarly to the existing systems without any degradation in \averageFalsePredictioins cases. 
\Name shows up to three orders of magnitude improvement in median 5G handover completion time for latency-sensitive apps~(\S\ref{sec:app_aware_control_plane_processing}).  

\noindent\textbf{Contributions:} In summary, we make the following contributions to this work: 
\begin{enumerate}[leftmargin=*]
\item We identify the key architectural bottlenecks in enabling stateful mobile applications over 5G (\S\ref{challenges}).
\item We design a new system architecture, \Name. \Name consists of three new modules for speeding up application handovers (\S\ref{sec:design}).
\item We implement \Name. Our implementation consists of a target base station predictor as well as an extended edge data store, on top of Redis and Memcached~(\S\ref{sec:implementation}).
\item We evaluate \Name with two real edge apps, CarMap, and EMP, and also perform a sensitivity analysis using a simulation framework (\S\ref{sec:evaluation}).
\end{enumerate}
% \begin{itemize}[leftmargin=*]
%     \item Design of a target BS prediction module.
%     \item Design of an edge data store to support faster App handover during mobility.
%     \item Design of an App-aware 5G control plane.
%     \item An implementation of the above modules.
% \end{itemize}


==> intro_v1.tex <==
% \vspace{-0.1in}
\section{Introduction}
5G and next-generation cellular networks aim to support emerging latency-sensitive applications (apps), such as safety apps for connected and autonomous vehicles~\cite{ahmad_carmap, zhang2021emp, infra_structure_assisted_car_map}, virtual and augmented reality (AR/VR) \cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}, edge-based video analytics~\cite{killer_app_edge_computing}, and multi-player online gaming \cite{online_gamming_delay_budget,zhang2017towards_online_game_updates_rate}. These apps place new demands of ultra-low latency on the 5G infrastructure, e.g., VR apps with head tracking systems require latency of less than 17ms to achieve perceptual stability~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

To reduce end-to-end delays and enable such apps, 5G networks are integrating Edge Computing~\cite{ar_vr_satyanarayanan2017emergence,mec_in_5g}; a paradigm whereby apps are hosted closer to the users, on cell towers, cell aggregation sites, or other edge sites~\cite{mec_in_5g, etsi2, etsi3}. Many cellular providers are partnering with cloud providers for deploying edge apps inside the cellular infrastructure~\cite{azure_edgezone, aws_wavelength, google_carriers}.  

Hosting apps at the network edge can significantly reduce delays. However, it also makes it challenging to ensure that users always receive low latency as they move across different locations. This in turn requires support to handover clients to different edge sites with negligible delays~\cite{mec_app_mobility_api_021}.
These app handovers are likely to be frequent~\cite{frequent_handover_zhou20215g, frequent_migration_abouaomar2021deep,  driving_frequent_app_handoverr,mec_in_5g, mec_evolution_toward_5g_etsi, etsi2} for a significant fraction of 5G use cases as more than 50\% of 5G IoTs are expected to be highly mobile apps related to the automotive industry \cite{5g_edge_computing_aws_53p}.\footnote{5G networks will have 5 billion connected IoTs by 2025~\cite{iot_in_5g_era_cisco}.} 
Many of these edge apps are stateful~\cite{zhang2021emp, ahmad_carmap, zhang2017towards_online_game_updates_rate, shi2019mobile_edge_vr, full_body_tracking_vr} and migrating stateful apps over 5G can cause significant app downtime during mobility~\cite{vm_container_migration_in_5g_mec,live_migration_yang2021multitier} (\S\ref{sec:slow_app_handover}). Consequently, if the app downtime exceeds the delay budget for latency-sensitive apps, it can compromise user safety in the case of connected cars~\cite{zhang2021emp, ahmad_carmap} or cause users motion sickness when using immersive mobile VR~\cite{motion_sickness_kundu2021study}.


In this paper, we first step back and ask the question, \textit{what are the key architectural bottlenecks in enabling stateful mobile edge apps over 5G}? We identify three key issues in enabling fast app handovers during mobility (illustrated in Figure~\ref{fig:challnges_serialized_ho}):


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/app_handover_challenges_contributions.png}
\vspace{-0.3in}
\caption{Key issues and possible directions to reduce downtime during app handover due to mobility. 5G handover delays range between 87-170\,ms~\cite{understanding_operational_5g} whereas session migration for edge apps takes atleast 140\,ms with existing techniques~(\S\ref{sec:slow_state_migration}).}
\label{fig:challnges_serialized_ho}
\vspace{-0.15in}
\end{figure}


\begin{itemize}[leftmargin=*]
\item \textbf{Uncoordinated and Reactive App Session Migration:} Stateful app handover involves two steps: (i)  migrating the user's network session, consisting of a 5G handover and, in some cases, Protocol Data Unit (PDU) session migration~\cite{pdu_session_establishment}, and (ii) migrating the user's app session. Uncoordinated migration of the network and app sessions can cause extended app downtime (Figure \ref{fig:challnges_serialized_ho}a). If app session migration occurs after a 5G handover, it can result in two interruptions: one during the 5G handover and another during app session migration. This is particularly problematic for latency-sensitive edge apps with highly dynamic states~\cite{zhang2017towards_online_game_updates_rate} that receive limited benefits from proactive state migration. In a coordinated app handover, where the interruption time for the 5G handover and app session migration overlap, the decision of \textit{when} and \textit{where} (to which target edge host) to perform the app handover depends on the 5G handover decision and target BS selection, respectively. Even with perfectly synchronized 5G handover and app session migration events~(Figure~\ref{fig:challnges_serialized_ho}b), app downtime can still exceed the delay budgets of latency-sensitive edge apps, typically around 10ms~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.


\item \textbf{Slow App Session Migration:} A key challenge with speeding up session migration of stateful apps is that they typically require the user's up-to-date app state at the target edge host before a user connects to it~\cite{harchol2018cessna}. However, existing techniques for app session migration are either slow~\cite{live_migration_8000803,vm_container_migration_in_5g_mec, hardware_accelerated_live_migration,efficient_container_migration,live_migration_269357, criu} or they implement app-specific optimizations~\cite{fast_check_point_recovery} which cannot be generalized (\S\ref{sec:slow_state_migration}). A key challenge is to design a session migration technique that is \textit{fast} and \textit{generic}. 

\item \textbf{App-agnostic 5G Handover:}
We observe that even if we somehow address the issue of slow app session migration, the time required for a 5G handover can become a bottleneck in enabling latency-sensitive edge apps, as shown in Figure~\ref{fig:challnges_serialized_ho}c (\S\ref{sec:app_agnostic_5g_handover}). 
An architectural issue is that 5G control plane processing is \textit{app-agnostic} and there are no 5G interfaces through which edge apps can inform the cellular control plane of their latency requirements.

\end{itemize}

To address the above issues, we propose a new system architecture, \Name (\underline{EdgeCat}alyst), for edge apps over 5G. \Name is a cross-layer design that (a) leverages the interfaces exposed by the Multi-access Edge Computing (MEC) framework in 5G~\cite{mec_in_5g} to share radio network information with edge apps so they can proactively perform app state migration, and (b) proposes new interfaces to share app's latency requirements with the 5G control plane for speeding up 5G handovers. \Name consists of the following key ideas:


\begin{itemize}[leftmargin=*]
    
\item \textbf{Target BS Prediction:}
To minimize app downtimes, a coordinated and proactive approach to app handovers is crucial. In order to achieve this, \Name predicts the target BS for a 5G handover in advance, allowing edge apps to initiate app state migration proactively (Figure \ref{fig:challnges_serialized_ho}c). While predicting 5G handovers is relatively easy~\cite{hassan2022vivisecting}, predicting the target BS presents challenges due to an average of 7.45 BSs available during a handover (\S\ref{sec:challenges:reactive_app_session_migration}).

Existing techniques for target BS prediction rely on handover history~\cite{bs_prediction_ho_history, bs_prediction_low_accuracy_3}, LTE events~\cite{bs_prediction_low_accuracy_1}, or machine learning approaches~\cite{bs_prediction_low_accuracy_2, bs_prediction_low_accuracy_4, bs_prediction_radio_link_characteristics}. However, the 5G network-based approaches have two common limitations: (i) they lack early prediction timing, which is crucial for practical benefits, as predicting the target BS only milliseconds before a handover provides negligible performance gains (\S\ref{sec:eval:impact_of_mobility_hint}), and (ii) their prediction accuracy is generally poor, ranging from 65\% to 85\%.

To overcome these limitations, we propose an early target BS prediction model based on a Long Short-Term Memory (LSTM) neural network. Our model utilizes data exposed by the Radio Network Information (RNI) APIs in MEC~\cite{5g_mec_rni1} (\S\ref{sec:design:target_bs_predction}), which includes radio information about mobile clients. We train and test our model using multiple real 5G/4G radio network traces, including data collected during driving tests~\cite{incp_dataset}, high-speed trains~\cite{li2020beyond}, and various other mobility scenarios \cite{mobile_insight_logs}. On average, our model accurately predicts \averageAccuracy of the target BSs  100 ms ahead of an actual handover (\S\ref{sec:eval:target_BS_prediction}). We refer to this advanced target base prediction as a "mobility hint" for apps.






\item \textbf{Two-Step App State Synchronization:}
An app can proactively synchronize all or a subset of the user's app state with the target edge host based on mobility hint. However, synchronizing a highly dynamic state object that is frequently updated offers little advantage as it quickly becomes stale. Additionally, identifying and tracking different types of state objects for proactive synchronization is a daunting task for developers. Instead, we propose extending existing data stores (e.g., \redis~\cite{redis_store} and \memcache~\cite{memcached_store}) to store and track the app state of an edge app. This extension allows us to track the update rate for each state object of an edge app~(\S\ref{sec:design_app_state_migration}). The server side of edge apps stores the per-user app state in our modified external data store, which exposes new APIs to edge apps~(Table~\ref{tab:api_in_edge_store}). These APIs enable the synchronization of state objects with low update rates upon receiving a mobility hint, and the remaining dynamic app state is synchronized during a 5G handover. This approach reduces blocking time during state migration, resulting in minimized app downtime~(\S\ref{sec:state_migration_delay}).


\item \textbf{App-Aware Control Plane Processing:}
To make 5G control plane processing app-aware, we introduce new APIs (Table \ref{tab:api_for_app_influence_on_cpf}) that allow edge apps to report their latency requirements and prioritize control plane processing accordingly (\S\ref{sec:app_impact_on_control_plane}). These APIs are called by the server side of latency-sensitive apps through the MEC \cite{mec_in_5g}, which influences control plane processing. Restricting API access to the server side ensures better control and prevents misuse, as it is under the network operator's control or managed by trusted third parties. Our experiments demonstrate that an app-aware 5G control plane significantly reduces handover delays, bringing edge app downtime within their specified delay budgets (\S\ref{sec:app_aware_control_plane_processing}).

\end{itemize}

To show the efficacy of the above ideas, we implement \Name. We implement the target BS prediction module using an 8-layer LSTM neural network on top of the Keras library~\cite{keras_library}. Our data sets consist of real 4G/5G traces with a total of \totalHandovers handovers. On the app layer, we implement dynamic state tracking and two-step state synchronization in \redis~\cite{redis_store} and \memcache~\cite{memcached_store} data stores~(\S\ref{sec:design_app_state_migration}). To evaluate the impact of \Name on real edge apps, we modify two recent open-source edge apps, CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}, to use our modified \redis data store for proactive state synchronization. As real apps provide limited options to vary app state properties (e.g., state sizes, update rate, etc.), we implement a simulation framework in Python to simulate the behavior of a wide variety of latency-sensitive edge apps~(\S\ref{sec:imp_modified_state_store}). We interface a Python version of both modified \memcache and \redis key-value data stores with the simulation framework to evaluate the impact of two-step state syncing on a wide variety of app behaviors. To implement app-aware control plane processing, we modify a recently proposed cellular control plane~\cite{neutrino_ton}. We provide further details of our implementations in \S\ref{sec:implementation}. We open-source our code on an anonymous Github link: \href{\repourl}{\repourl}.

Our evaluation shows up to $14\times$ and $15.4\times$ improvement in app downtime for CarMap and EMP, respectively. \Name on average correctly predicts \averageAccuracy of the target BSs 100\,ms ahead of an actual handover (\S\ref{sec:eval:impact_of_mobility_hint}). Consequently, CarMap and EMP show more than $3\times$ and $2.5\times$ improvement in app state migration time, respectively~(\S\ref{sec:state_migration_delay}). 
% \Name significantly improves app state migration time in \averageAccuracy cases with correct BSs predictions or performs similarly to the existing systems without any degradation in \averageFalsePredictioins cases. 
\Name shows up to three orders of magnitude improvement in median 5G handover completion time for latency-sensitive apps~(\S\ref{sec:app_aware_control_plane_processing}).  

\noindent\textbf{Contributions:} In summary, we make the following contributions to this work: 
\begin{enumerate}[leftmargin=*]
\item We identify the key architectural bottlenecks in enabling stateful mobile apps over 5G (\S\ref{challenges}).
\item We design a new system architecture, \Name. \Name consists of three new modules for speeding up app handovers (\S\ref{sec:design}).
\item We implement \Name. Our implementation consists of a target BS predictor as well as an extended edge data store, on top of Redis and Memcached~(\S\ref{sec:implementation}).
\item We evaluate \Name with two real edge apps, CarMap, and EMP, and also perform a sensitivity analysis using a simulation framework (\S\ref{sec:evaluation}).
\end{enumerate}
% \begin{itemize}[leftmargin=*]
%     \item Design of a target BS prediction module.
%     \item Design of an edge data store to support faster App handover during mobility.
%     \item Design of an App-aware 5G control plane.
%     \item An implementation of the above modules.
% \end{itemize}


==> intro_v2.tex <==
% \vspace{-0.1in}
\section{Introduction}
5G and next-generation cellular networks aim to support emerging latency-sensitive applications (apps), such as safety apps for connected and autonomous vehicles~\cite{ahmad_carmap, zhang2021emp, infra_structure_assisted_car_map}, virtual and augmented reality (AR/VR) \cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}, edge-based video analytics~\cite{killer_app_edge_computing}, and multi-player online gaming \cite{online_gamming_delay_budget,zhang2017towards_online_game_updates_rate}. These apps place new demands of ultra-low latency on the 5G infrastructure, e.g., VR apps with head tracking systems require latency of less than 17ms to achieve perceptual stability~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

To reduce end-to-end delays and enable such apps, 5G networks are integrating Edge Computing~\cite{ar_vr_satyanarayanan2017emergence,mec_in_5g}; a paradigm whereby apps are hosted closer to the users, on cell towers, cell aggregation sites, or other edge sites~\cite{mec_in_5g, etsi2, etsi3}. Many cellular providers are partnering with cloud providers for deploying edge apps inside the cellular infrastructure~\cite{azure_edgezone, aws_wavelength, google_carriers}.  

Hosting apps at the network edge can significantly reduce delays. However, it also makes it challenging to ensure that users always receive low latency as they move across different locations. This in turn requires support to handover clients to different edge sites with negligible delays~\cite{mec_app_mobility_api_021}.
These app handovers are likely to be frequent~\cite{frequent_handover_zhou20215g, frequent_migration_abouaomar2021deep,  driving_frequent_app_handoverr,mec_in_5g, mec_evolution_toward_5g_etsi, etsi2} for a significant fraction of 5G use cases as more than 50\% of 5G IoTs are expected to be highly mobile apps related to the automotive industry \cite{5g_edge_computing_aws_53p}.\footnote{5G networks will have 5 billion connected IoTs by 2025~\cite{iot_in_5g_era_cisco}.} 
Many of these edge apps are stateful~\cite{zhang2021emp, ahmad_carmap, zhang2017towards_online_game_updates_rate, shi2019mobile_edge_vr, full_body_tracking_vr} and migrating stateful apps over 5G can cause significant app downtime during mobility~\cite{vm_container_migration_in_5g_mec,live_migration_yang2021multitier} (\S\ref{sec:slow_app_handover}). Consequently, if the app downtime exceeds the delay budget for latency-sensitive apps, it can compromise user safety in the case of connected cars~\cite{zhang2021emp, ahmad_carmap} or cause users motion sickness when using immersive mobile VR~\cite{motion_sickness_kundu2021study}.


In this paper, we first step back and ask the question, \textit{what are the key architectural bottlenecks in enabling stateful mobile edge apps over 5G}? We identify three key issues in enabling fast app handovers during mobility (illustrated in Figure~\ref{fig:challnges_serialized_ho}):


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/app_handover_challenges_contributions.png}
\vspace{-0.3in}
\caption{Key issues and possible directions to reduce downtime during app handover due to mobility. 5G handover delays range between 87-170\,ms~\cite{understanding_operational_5g} whereas session migration for edge apps takes atleast 140\,ms with existing techniques~(\S\ref{sec:slow_state_migration}).
% \zafar{This figure has become a bit complicated and hence difficult to understand. Lets discuss if we can simplify it. One option is to simplify the (d) subfigure by removing the additional annotations, i.e., proactive state migration and prioritized handover and then we can consider if we want a separate small figure (later on) to explain this. Please make the (a) to (d) subfigure titles bold so they stand out. We can also move the time horizontal at the top, line along with legend, and make the line smaller. Another minor point, in the legend since we are using the abbreviation App, we should say App Downtime and App Delay Budget.}
}
\label{fig:challnges_serialized_ho}
\vspace{-0.2in}
\end{figure}


\begin{itemize}[leftmargin=*]
\item \textbf{Uncoordinated and Reactive App Session Migration:} Stateful app handover involves two key steps: (i) the user's network session migration (5G handover\footnote{A 5G or base station (BS) handover might also trigger Packet Data Unit (PDU) session migration~\cite{3gpp_123_502,pdu_session_establishment}.}) and (ii) the user's app session migration. Uncoordinated migration of the network and app sessions can cause extended app downtime (Figure \ref{fig:challnges_serialized_ho}a). If app session migration occurs after a 5G handover, it can result in two interruptions: one during the 5G handover and another during app session migration.
This can be particularly a concern for latency-sensitive edge apps with highly dynamic app state~\cite{zhang2017towards_online_game_updates_rate} where even a proactive session migration would result in a non-zero downtime.
% This is particularly problematic for latency-sensitive edge apps with highly dynamic states~\cite{zhang2017towards_online_game_updates_rate} that receive limited benefits from proactive state migration. 
In a coordinated app handover, where the interruption time for the 5G handover and app session migration overlap, the decision of \textit{when} and \textit{where} (to which target edge host) to perform the app handover depends on the 5G handover decision and target BS selection, respectively. Even with perfectly synchronized 5G handover and app session migration events~(Figure~\ref{fig:challnges_serialized_ho}b), app downtime can still exceed the delay budgets of latency-sensitive edge apps, which is typically around 10~ms~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.


\item \textbf{Slow App Session Migration:} A key challenge with speeding up session migration of stateful apps is that they typically require the user’s up-to-date app state at the target edge host before a user connects to it~\cite{harchol2018cessna}. However, existing techniques for app session migration are either slow~\cite{live_migration_8000803, vm_container_migration_in_5g_mec, hardware_accelerated_live_migration, efficient_container_migration, live_migration_269357, criu} or rely on app-specific optimizations~\cite{fast_check_point_recovery}~(\S\ref{sec:slow_state_migration}). 
% Moreover, simpler session migration techniques, such as continuing the session with the source app instance before state migration completes, can result in two interruptions: one during the 5G handover and another during app session migration. 
% This occurs because the app session at the source edge host needs to be frozen, migrated, and restarted on the target edge host to ensure state consistency.
The key challenge is to design a session migration technique that is \textit{fast} and \textit{generic}.

\item \textbf{App-agnostic 5G Handover:}
We observe that even if we somehow address the issue of slow app session migration, the time required for a 5G handover can become a bottleneck in enabling latency-sensitive edge apps, as shown in Figure~\ref{fig:challnges_serialized_ho}c (\S\ref{sec:app_agnostic_5g_handover}). 
An architectural issue is that 5G control plane processing is \textit{app-agnostic} and there are no 5G interfaces through which edge apps can inform the cellular control plane of their latency requirements.

\end{itemize}

To address the above issues, we propose a new system architecture, \Name (\underline{EdgeCat}alyst), for edge apps over 5G. \Name is a cross-layer design that (a) leverages the interfaces exposed by the Multi-access Edge Computing (MEC) framework in 5G~\cite{mec_in_5g} to share radio network information with edge apps so they can proactively perform app state migration, and (b) proposes new interfaces to share app's latency requirements with the 5G control plane for speeding up 5G handovers. \Name consists of the following key ideas:


\begin{itemize}[leftmargin=*]
    
\item \textbf{Target BS Prediction:}
To minimize app downtimes, a coordinated and proactive approach to app handovers is crucial. To achieve this, \Name predicts the target BS for a 5G handover in advance, allowing edge apps to initiate app state migration proactively (Figure \ref{fig:challnges_serialized_ho}c). While predicting handovers is relatively easy~\cite{hassan2022vivisecting}, predicting the target BS presents challenges due to transient fluctuations in radio signals, especially in mmWave-based 5G networks, and an average of 7.45 BSs available during a handover (\S\ref{sec:challenges:reactive_app_session_migration}).

Existing techniques for target BS prediction rely on handover history~\cite{bs_prediction_ho_history, bs_prediction_low_accuracy_3}, LTE events~\cite{bs_prediction_low_accuracy_1}, or machine learning approaches~\cite{bs_prediction_low_accuracy_2, bs_prediction_low_accuracy_4, bs_prediction_radio_link_characteristics}. However, the existing 5G network-based approaches have two common limitations: (i) they lack early prediction timing, which is crucial for practical benefits, as predicting the target BS only milliseconds before a handover provides negligible performance gains (\S\ref{sec:eval:impact_of_mobility_hint}), and (ii) their prediction accuracy is generally poor (< 85\%).

To overcome these limitations, we propose an early target BS prediction model based on a Long Short-Term Memory (LSTM) neural network. Our model utilizes data exposed by the Radio Network Information (RNI) APIs in MEC~\cite{5g_mec_rni1} (\S\ref{sec:design:target_bs_predction}), which includes radio information about mobile clients. We train and test our model using multiple real 5G/4G radio network traces, including data collected during driving tests~\cite{incp_dataset}, high-speed trains~\cite{li2020beyond}, and various other mobility scenarios \cite{mobile_insight_logs}. On average, our model accurately predicts \averageAccuracy of the target BSs  100 ms ahead of an actual handover (\S\ref{sec:eval:target_BS_prediction}). We refer to this advanced target base prediction as a "mobility hint" for apps.






\item \textbf{Two-Step App State Synchronization:}
An app can proactively synchronize all or a subset of the user's app state with the target edge host based on mobility hint. However, synchronizing a highly dynamic state object that is frequently updated offers little advantage as it quickly becomes stale. Additionally, identifying and tracking different types of state objects for proactive synchronization is a daunting task for developers. Instead, we propose extending existing data stores (e.g., \redis~\cite{redis_store} and \memcache~\cite{memcached_store}) to store and track the app state of an edge app. This extension allows us to track the update rate for each state object of an edge app~(\S\ref{sec:design_app_state_migration}). The server side of edge apps stores the per-user app state in our modified external data store. The modified data store exposes new APIs 
~(Table~\ref{tab:api_in_edge_store}) to edge apps to enable the synchronization of state objects with low update rates upon receiving a mobility hint, and the remaining app state is synchronized during a 5G handover to maximally overlap interruption time (Figure~\ref{fig:challnges_serialized_ho}c). This approach reduces blocking time during state migration, resulting in minimized app downtime~(\S\ref{sec:state_migration_delay}).


\item \textbf{App-Aware Control Plane Processing:}
To make 5G control plane processing app-aware, we introduce new APIs (Table \ref{tab:api_for_app_influence_on_cpf}) that allow edge apps to report their latency requirements and prioritize control plane processing accordingly (\S\ref{sec:app_impact_on_control_plane}). These APIs are called by the server side of latency-sensitive apps through the MEC \cite{mec_in_5g}, which influences control plane processing. Restricting API access to the server side ensures better control and prevents misuse, as it is under the network operator's control or managed by trusted third parties. Our experiments demonstrate that an app-aware 5G control plane significantly reduces handover delays, bringing edge app downtime within their specified delay budgets (\S\ref{sec:app_aware_control_plane_processing}).

\end{itemize}

To show the efficacy of the above ideas, we implement \Name. We implement the target BS prediction module using an 8-layer LSTM neural network on top of the Keras library~\cite{keras_library}. Our data sets consist of real 4G/5G traces with a total of \totalHandovers handovers. On the app layer, we implement dynamic state tracking and two-step state synchronization in \redis~\cite{redis_store} and \memcache~\cite{memcached_store} data stores~(\S\ref{sec:design_app_state_migration}). To evaluate the impact of \Name on real edge apps, we modify two recent open-source edge apps, CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}, to use our modified \redis data store for proactive state synchronization. As real apps provide limited options to vary app state properties (e.g., state sizes, update rate, etc.), we implement a simulation framework in Python to simulate the behavior of a wide variety of latency-sensitive edge apps~(\S\ref{sec:imp_modified_state_store}). We interface a Python version of both modified \memcache and \redis key-value data stores with the simulation framework to evaluate the impact of two-step state syncing on a wide variety of app behaviors. To implement app-aware control plane processing, we modify a recently proposed cellular control plane~\cite{neutrino_ton}. We provide further details of our implementations in \S\ref{sec:implementation}. We open-source our code on an anonymous Github link: \href{\repourl}{\repourl}.

Our evaluation shows up to $14\times$ and $15.4\times$ improvement in app downtime for CarMap and EMP, respectively. \Name on average correctly predicts \averageAccuracy of the target BSs 100\,ms ahead of an actual handover (\S\ref{sec:eval:impact_of_mobility_hint}). Consequently, CarMap and EMP show more than $3\times$ and $2.5\times$ improvement in app state migration time, respectively~(\S\ref{sec:state_migration_delay}). 
% \Name significantly improves app state migration time in \averageAccuracy cases with correct BSs predictions or performs similarly to the existing systems without any degradation in \averageFalsePredictioins cases. 
\Name shows up to three orders of magnitude improvement in median 5G handover completion time for latency-sensitive apps~(\S\ref{sec:app_aware_control_plane_processing}).  

\noindent\textbf{Contributions:} In summary, we make the following contributions to this work: 
\begin{enumerate}[leftmargin=*]
\item We identify the key architectural bottlenecks in enabling stateful mobile apps over 5G (\S\ref{challenges}).
\item We design a new system architecture, \Name. \Name consists of three new modules for speeding up app handovers (\S\ref{sec:design}).
\item We implement \Name. Our implementation consists of a target BS predictor as well as an extended edge data store, on top of Redis and Memcached~(\S\ref{sec:implementation}).
\item We evaluate \Name with two real edge apps, CarMap, and EMP, and also perform a sensitivity analysis using a simulation framework (\S\ref{sec:evaluation}).
\end{enumerate}
% \begin{itemize}[leftmargin=*]
%     \item Design of a target BS prediction module.
%     \item Design of an edge data store to support faster App handover during mobility.
%     \item Design of an App-aware 5G control plane.
%     \item An implementation of the above modules.
% \end{itemize}



==> intro_v3.tex <==
% \vspace{-0.1in}
\section{Introduction}
5G and next-generation cellular networks aim to support emerging latency-sensitive applications (apps), such as safety apps for connected and autonomous vehicles~\cite{ahmad_carmap, zhang2021emp, infra_structure_assisted_car_map}, virtual and augmented reality (AR/VR) \cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}, edge-based video analytics~\cite{killer_app_edge_computing}, and multi-player online gaming \cite{online_gamming_delay_budget,zhang2017towards_online_game_updates_rate}. These apps place new demands of ultra-low latency on the 5G infrastructure, e.g., VR apps with head tracking systems require latency of less than 17ms to achieve perceptual stability~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}.

To reduce end-to-end delays and enable such apps, 5G networks are integrating Edge Computing~\cite{ar_vr_satyanarayanan2017emergence,mec_in_5g}; a paradigm whereby apps are hosted closer to the users, on cell towers, cell aggregation sites, or other edge sites~\cite{mec_in_5g, etsi2, etsi3}. Many cellular providers are partnering with cloud providers for deploying edge apps inside the cellular infrastructure~\cite{azure_edgezone, aws_wavelength, google_carriers}.  

Hosting apps at the network edge can significantly reduce delays. However, it also makes it challenging to ensure that users always receive low latency as they move across different locations. This, in turn, requires support to handover clients to different edge sites with negligible delays~\cite{mec_app_mobility_api_021}.
These app handovers are likely to be frequent~\cite{frequent_handover_zhou20215g, frequent_migration_abouaomar2021deep,  driving_frequent_app_handoverr,mec_in_5g, mec_evolution_toward_5g_etsi, etsi2} for a significant fraction of 5G use cases as more than 50\% of 5G IoTs are expected to be highly mobile apps related to the automotive industry \cite{5g_edge_computing_aws_53p}.\footnote{5G networks will have 5 billion connected IoTs by 2025~\cite{iot_in_5g_era_cisco}.} 
Many of these edge apps are stateful~\cite{zhang2021emp, ahmad_carmap, zhang2017towards_online_game_updates_rate, shi2019mobile_edge_vr, full_body_tracking_vr} and migrating stateful apps over 5G can cause significant app downtime during mobility~\cite{vm_container_migration_in_5g_mec,live_migration_yang2021multitier} (\S\ref{sec:slow_app_handover}). Consequently, if the app downtime exceeds the delay budget for latency-sensitive apps, it can compromise user safety in the case of connected cars~\cite{zhang2021emp, ahmad_carmap} or cause users motion sickness when using immersive mobile VR~\cite{motion_sickness_kundu2021study}.


In this paper, we first step back and ask the question, \textit{what are the key architectural bottlenecks in enabling stateful mobile edge apps over 5G}? We identify three key issues in enabling fast app handovers during mobility (illustrated in Figure~\ref{fig:challnges_serialized_ho}):


\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/app_handover_challenges_contributions.png}
\vspace{-0.3in}
\caption{Key issues and possible directions to reduce downtime during app handover due to mobility. 5G handover delay 87 to 170\,ms~\cite{understanding_operational_5g} \& app session migration delay >140\,ms with existing techniques~(\S\ref{sec:slow_state_migration}).
}
\label{fig:challnges_serialized_ho}
\vspace{-0.2in}
\end{figure*}


\begin{itemize}[leftmargin=*]
\item \textbf{Uncoordinated and Reactive App Session Migration:} Stateful app handover involves two key steps: (i) the user's network session migration, also known as 5G handover\footnote{A 5G handover can also trigger user plane session migration---referred to as Packet Data Unit session migration~\cite{3gpp_123_502,pdu_session_establishment}).} and (ii) the user's app session migration. Uncoordinated migration of the network and app sessions can cause extended app downtime (Figure \ref{fig:challnges_serialized_ho}a). If the app session migration occurs after a 5G handover, it can result in two interruptions, one during the 5G handover and another during the app session migration. Even if app session migration is performed proactively, latency-sensitive apps that frequently update app state~\cite{zhang2017towards_online_game_updates_rate} can incur non-zero downtime to retrieve the latest app state. %For latency-sensitive apps that frequently update app state~\cite{zhang2017towards_online_game_updates_rate}, a challenge is that even if they proactively perform app session migration, it can result in non-zero downtime.
%This can be particularly problematic for latency-sensitive edge apps that frequently update app state~\cite{zhang2017towards_online_game_updates_rate}, where even proactive app session migration can result in non-zero app downtime. 
%If app session migration occurs after a 5G handover, it can result in two interruptions: one during the 5G handover and another during app session migration.
%This can be particularly problematic where even proactive app session migration would result in a non-zero app downtime, i.e., latency-sensitive edge apps with app state frequently updated~\cite{zhang2017towards_online_game_updates_rate}.
% This can be particularly a concern for latency-sensitive edge apps with app state frequently updated~\cite{zhang2017towards_online_game_updates_rate} where even a proactive session migration would result in a non-zero downtime.
% This is particularly problematic for latency-sensitive edge apps with highly dynamic states~\cite{zhang2017towards_online_game_updates_rate} that receive limited benefits from proactive state migration. 
%In a coordinated app handover, where the interruption time for the 5G handover and app session migration overlap, the decision of \textit{when} and \textit{where} (to which target edge host) to perform the app handover depends on the 5G handover decision and target BS selection, respectively. 
On the other hand, even if we perfectly synchronize 5G handover and app session migration events~(Figure~\ref{fig:challnges_serialized_ho}b), app downtime can still exceed the delay budget~(<~17\,ms~\cite{elbamby2018toward, ar_vr_satyanarayanan2017emergence}) of latency-sensitive edge apps.


\item \textbf{Slow App Session Migration:} A key challenge with speeding up session migration of stateful apps is that they typically require the user’s up-to-date app state at the target edge host before a user connects to it~\cite{harchol2018cessna}. However, existing techniques for app session migration are either slow~\cite{live_migration_8000803, vm_container_migration_in_5g_mec, hardware_accelerated_live_migration, efficient_container_migration, live_migration_269357, criu} or rely on app-specific optimizations~\cite{fast_check_point_recovery}~(\S\ref{sec:slow_state_migration}). 
Moreover, simpler session migration techniques, such as continuing the app session with the source instance before state migration completes, can result in two interruptions: one during the 5G handover and another during app session migration. 
This occurs because the app session at the source edge host needs to be frozen, migrated, and restarted on the target edge host to ensure state consistency.
The key challenge is to design a session migration technique that is \textit{fast} and \textit{generic}.

\item \textbf{App-agnostic 5G Handover:}
We observe that even if we somehow address the issue of slow app session migration, the time required for a 5G handover can become a bottleneck in enabling latency-sensitive edge apps, as shown in Figure~\ref{fig:challnges_serialized_ho}c (\S\ref{sec:app_agnostic_5g_handover}). 
An architectural issue is that 5G control plane processing is \textit{application-agnostic} and there are no 5G interfaces through which edge apps can inform the cellular control plane of their latency requirements.

\end{itemize}

To address the above issues, we propose a new system architecture, \Name (\underline{EdgeCat}alyst), for edge apps over 5G. \Name is a cross-layer design that consists of the following key ideas: %that (a) leverages the interfaces exposed by the Multi-access Edge Computing (MEC) framework in 5G~\cite{mec_in_5g} to share radio network information with edge apps so they can proactively perform app state migration, and (b) proposes new interfaces to share app's latency requirements with the 5G control plane for speeding up 5G handovers. \Name consists of the following key ideas:


\begin{itemize}[leftmargin=*]
    
\item \textbf{Target BS Prediction:}
A coordinated and proactive approach to app handovers is essential for minimizing app downtimes. To achieve this, \Name predicts the target BS\footnote{Predicting the target BS is equivalent to predicting the target edge host as it is a function of target BS. Details in \S\ref{sec:goals_and_assumptions}.} for a 5G handover in advance, allowing edge apps to initiate app state migration proactively (Figure \ref{fig:challnges_serialized_ho}c). 
Existing techniques for target BS prediction
rely on handover history~\cite{bs_prediction_ho_history, bs_prediction_low_accuracy_3}, LTE events~\cite{bs_prediction_low_accuracy_1}, or machine learning approaches~\cite{bs_prediction_low_accuracy_2, bs_prediction_low_accuracy_4, bs_prediction_radio_link_characteristics}. Among these, the 5G network-based approaches have two common limitations: (i) they lack early prediction timing, which is crucial for practical benefits, as predicting the target BS only a few milliseconds before a handover provides negligible performance gains (\S\ref{sec:eval:impact_of_mobility_hint}), and (ii) their prediction accuracy is generally poor (< 85\%).

To overcome these limitations, we propose a multi-step early target BS prediction pipeline (\S\ref{sec:design:target_bs_predction}), which leverages Radio Network Information (RNI) APIs in MEC~\cite{5g_mec_rni1} to predict handovers in advance using an LSTM network, then extrapolate radio measurements to enable early target BS prediction, and finally perform target BS prediction.
We evaluate this pipeline on real 5G/4G radio network traces, including data from driving tests~\cite{incp_dataset}, high-speed trains~\cite{li2020beyond}, and various other mobility scenarios~\cite{mobile_insight_logs}. Our evaluation shows on average \averageAccuracy correct 
 predictions of the target BS 100 ms ahead of the handover~(\S\ref{sec:eval:target_BS_prediction}), which we refer to as a \textit{mobility hint} for apps.
Our approach outperforms existing techniques, including LSTM-based networks~\cite{bs_prediction_low_accuracy_4}, by leveraging (i) enhanced feature vectors (\S\ref{appendix_feature_vector}) capturing time-series radio signal trends and (ii)
extrapolation of radio signals (\S\ref{sec:design:target_bs_predction}) when sample data is insufficient.
 
% Our approach significantly outperforms the existing techniques, including LSTM-based networks~\cite{bs_prediction_low_accuracy_4}, due to (i) the composition of the feature vector(~\S\ref{appendix_feature_vector}) that captures time-series trends in the radio signals, and (ii) radio signals extrapolation when enough samples are not received~(\S\ref{sec:design:target_bs_predction}).



\item \textbf{Two-Step App State Synchronization:}
An app can proactively synchronize all or a subset of the user's app state with the target edge host based on mobility hint. However, synchronizing a highly dynamic state object that is frequently updated offers little advantage as it quickly becomes stale. Additionally, identifying and tracking different types of state objects for proactive synchronization is a daunting task for developers. Instead, we propose extending existing edge data stores (e.g., \redis~\cite{redis_store} and \memcache~\cite{memcached_store}) to store and track the app state of an edge app. This extension allows us to track the update rate for each state object of an edge app~(\S\ref{sec:design_app_state_migration}). The server side of edge apps stores the per-user (in-memory) app state in our modified external data store. The modified data store exposes new APIs 
~(Table~\ref{tab:api_in_edge_store}) to edge apps to enable the synchronization of state objects with low update rates upon receiving a mobility hint, and the remaining app state is synchronized during a 5G handover to maximally overlap interruption time (Figure~\ref{fig:challnges_serialized_ho}c). This approach reduces blocking time during state migration, resulting in minimized app downtime~(\S\ref{sec:state_migration_delay}).


\item \textbf{App-Aware Control Plane Processing:}
To make 5G control plane processing app-aware, we introduce new APIs (Table \ref{tab:api_for_app_influence_on_cpf}) that allow edge apps to report their latency requirements and prioritize control plane processing accordingly (\S\ref{sec:app_impact_on_control_plane}). These APIs are called by the server side of latency-sensitive apps through the MEC \cite{mec_in_5g}, which influences control plane processing. Restricting API access to the server side ensures better control and prevents misuse, as it is under the network operator's control or managed by trusted third parties. Our experiments demonstrate that an app-aware 5G control plane significantly reduces handover delays, bringing edge app downtime within their specified delay budgets (\S\ref{sec:app_aware_control_plane_processing}).

\end{itemize}

To show the efficacy of the above ideas, we implement \Name. We implement a multi-step target BS prediction pipeline utilizing an 8-layer stacked LSTM neural network on top of Keras library~\cite{keras_library}. Our data sets consist of real 4G/5G traces with a total of \totalHandovers handovers. On the app layer, we implement dynamic state tracking and two-step state synchronization in \redis~\cite{redis_store} and \memcache~\cite{memcached_store} data stores~(\S\ref{sec:design_app_state_migration}). To evaluate the impact of \Name on real edge apps, we modify two recent open-source edge apps, CarMap~\cite{ahmad_carmap} and EMP~\cite{zhang2021emp}, to use our modified \redis data store for proactive state synchronization. As real apps provide limited options to vary app state properties (e.g., state sizes, update rate, etc.), we implement a simulation framework in Python to simulate the behavior of a wide variety of latency-sensitive edge apps~(\S\ref{sec:imp_modified_state_store}). We interface a Python version of both modified \memcache and \redis key-value data stores with the simulation framework to evaluate the impact of two-step state syncing on a wide variety of app behaviors. To implement app-aware control plane processing, we modify a recently proposed cellular control plane~\cite{neutrino_ton}. We provide further details of our implementations in \S\ref{sec:implementation}. We open-source our code on an anonymous Github link: \href{\repourl}{\repourl}.

Our evaluation shows up to $14\times$ and $15.4\times$ improvement in app downtime for CarMap and EMP, respectively.
We correctly predict the target BS in \averageAccuracy cases at least 100\,ms in advance, in \averageFalsePredictioins cases less than 100\,m       s in advance, and fail to predict the correct target BS in \noPredictionAvaragePercentage cases. Apps can significantly improve performance during mobility with correct target BS predictions (Figure \S\ref{fig:challnges_serialized_ho}c), while neither improving nor degrading performance in the case of false predictions due to fallback on reactive migration (Figure \S\ref{fig:challnges_serialized_ho}b).
Consequently, CarMap and EMP show more than $3\times$ and $2.5\times$ improvement in app state migration time, respectively~(\S\ref{sec:state_migration_delay}). 
\Name shows up to $10^3\times$ improvement in median 5G handover completion time for latency-sensitive apps~(\S\ref{sec:app_aware_control_plane_processing}).  

\noindent\textbf{Contributions:} In summary, we make the following contributions to this work: 
\begin{enumerate}[leftmargin=*]
\item We identify the key architectural bottlenecks in enabling stateful mobile apps over 5G (\S\ref{challenges}).
\item We design a new system architecture, \Name, compatible with RAN and cellular core (e.g., 5G/4G/LTE). \Name consists of three new modules to speed up app handovers (\S\ref{sec:design}).
\item We implement \Name. Our implementation consists of a target BS predictor, an extended edge data store on top of Redis and Memcached, and an app-aware 5G control plane (\S\ref{sec:implementation}).
\item We evaluate \Name with two real edge apps, CarMap, and EMP, with multiple real-world cellular data sets, and also perform a sensitivity analysis using a simulation framework (\S\ref{sec:evaluation}).
\end{enumerate}
% \begin{itemize}[leftmargin=*]
%     \item Design of a target BS prediction module.
%     \item Design of an edge data store to support faster App handover during mobility.
%     \item Design of an App-aware 5G control plane.
%     \item An implementation of the above modules.
% \end{itemize}


==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\noindent\textbf{Target BS Prediction:}
In prior work~\cite{bs_prediction_radio_link_characteristics, bs_prediction_ho_history, bs_prediction_low_accuracy_1}, target BS prediction is performed using support vector machines, handover history, and LTE event patterns. However, these studies focused on pre-5G networks, which differ from 5G with mmWave having limited range and more susceptible to physical obstacles~\cite{5g_mmWave}. Recent 5G-based approaches employed deep neural networks~\cite{bs_prediction_low_accuracy_2}, historical handovers~\cite{bs_prediction_low_accuracy_3}, and LSTM networks~\cite{bs_prediction_low_accuracy_4}. Notably, all these methods lack early prediction timings and provide relatively low prediction accuracy (<85\%).

\noindent\textbf{Resilience, Placement, and Load Balancing at the Edge:} 
CESSNA \cite{harchol2018cessna} aims to guarantee consistent application state recovery in edge failures and client mobility scenarios. The design is based on message logging and periodic state check-pointing for failure recovery. Portkey ~\cite{noor2021portkey} aims to design a distributed key-value store that dynamically adapts data placement decisions based on the client's mobility and data access patterns. This design is based on passive profiling and active probing of the edge servers. EdgeBalance~\cite{zhang2020edgebalance} aims for load balancing of the edge apps. Its design is based on CPU load prediction and adaptive distribution of the server load. All these proposals can be used with our proposed design to further improve the edge apps' performance.

\noindent\textbf{Mobility Impact on Application Performance:}
A recent work~\cite{hassan2022vivisecting} quantifies the impact of mobility on app performance, power consumption, and signaling overheads. This work designs a \handover prediction module \textit{Prognos} and demonstrates its ability to improve real app performance. This work does not consider the problem of application session migration during mobility. In addition, this work does not speed up 5G handovers for latency-sensitive edge apps.

\noindent\textbf{Reducing Cellular Control Plane Latency:}
There are several recent cellular control plane designs~\cite{sigcomm22_l25gc,dpcm, cellclone, neutrino, mmlite,larrea2023corekube} to reduce control plane delays under normal and fault scenarios. L25GC~\cite{sigcomm22_l25gc} incorporates shared-memory communication, smart buffering at the UPF, and a fast failure recovery protocol. DPCM~\cite{dpcm} leverages the device-side state to accelerate control plane operations. Neutrino~\cite{neutrino} utilizes modified FlatBuffers~\cite{flat-buffers} to speed up control plane operations and implements a two-step fault recovery protocol. CellClone~\cite{cellclone} masks control plane faults with active control plane clones at the edge. MMLite~\cite{mmlite} proposes a functionally decomposed, stateless control plane design in which procedures are implemented as micro-services and the state is externalized. MMLite allows prioritizing specific procedures. However, it does not provide any interface for edge apps to dynamically influence their control plane processing while running a latency-sensitive data session. \textcolor{blue}{CoreKube~\cite{larrea2023corekube} is a message-focused stateless cellular core design providing scalability and resilience to failures.} These proposals are complementary and can further help in reducing cellular control plane latency. 



% L\textsuperscript{2}5GC~\cite{sigcomm22_l25gc} key ideas are shared-memory communication, smart buffering at the UPF, and fast failure recovery protocol. DPCM~\cite{dpcm} leverages the device side state to speed up control plane operations. Neutrino~\cite{neutrino} leverages modified FlatBuffers~\cite{flat-buffers} to speed up control plane operations and uses a two-level fault recovery protocol for fast failure recovery. CellClone~\cite{cellclone} masks control plane faults with active control plane clones at the edge. MMLite~\cite{mmlite} proposes a functionally decomposed, stateless control plane design in which procedures are implemented as micro-services and the state is externalized. MMLite allows prioritizing specific procedures. However, it does not provide any interface for edge apps to dynamically influence their control plane processing while running a latency-sensitive data session. These proposals are complementary and can further help in reducing cellular control plane latency.

% There are several recent proposals~\cite{neutrino,sigcomm22_l25gc,mmlite,dpcm} to reduce the time taken to complete cellular control plane operations. L\textsuperscript{2}5GC~\cite{sigcomm22_l25gc} re-architects the 5G core network to reduce control plane delays. Their key ideas are shared-memory communication, smart buffering at the UPF, and fast failure recovery protocol.
% MMLite~\cite{mmlite} proposes a functionally decomposed, stateless control plane design in which procedures are implemented as micro-services and the state is externalized. MMLite allows prioritizing specific procedures. However, it does not provide any interface for edge apps to dynamically influence their control plane processing while running a latency-sensitive data session. Neutrino~\cite{neutrino} leverages modified FlatBuffers~\cite{flat-buffers} to speed up control plane operations and uses a two-level fault recovery protocol for fast failure recovery. These proposals are complementary and can further help in reducing cellular control plane latency.
%All these proposals do not perform any priority-based control plane processing for latency-sensitive edge apps, which can further reduce control plane delays.

% \noindent\textbf{Reducing Cellular Control Plane Latency:}
% There are several recent proposals~\cite{dpcm, neutrino,sigcomm22_l25gc,mmlite} to reduce the time taken to complete cellular control plane operations. DPCM \cite{dpcm} leverages the devices' side state to speed up the control plane operations and handle transient radio failures. L\textsuperscript{2}5GC~\cite{sigcomm22_l25gc} re-architects the 5G core network to reduce control plane delays and their impact on applications. Their key ideas are shared-memory communication, smart buffering at the UPF, and fast failure recovery protocol.
% MMLite~\cite{mmlite} proposes a functionally decomposed stateless control plane design where procedures are implemented as micro-services and the state is externalized. MMLite allows prioritizing particular procedures over others. MMLite does not provide any interface to the edge apps to dynamically influence its control plane processing when running a latency-sensitive data session. Neutrino~\cite{neutrino} leverages modified FlatBuffers~\cite{flat-buffers} to speed up control plane operations and uses a two-level fault recovery protocol for fast failure recovery. 
% All these proposals do not perform any priority-based control plane processing for latency-sensitive edge applications, which can further reduce control plane delays.

==> to-do-list.tex <==
% \color{red}
% To-Do List:
% \begin{itemize}
%     \item Update experimental setup details. A laptop was used as a mobile client instead of a server.
%     \item It would be better to have a figure representing our testbed. We can explicitly say we have created a testbed.
%     \item Provide a more detailed and concise description of our deployment model.
%     \item Justify why our LSTM model works better than the rest.
%     \item For apps, CarMap and EMP, explain how reduction in downtime is beneficial for these applications.
% \end{itemize}

% \color{black}
